Clenshaw Graph Neural Networks

Graph Convolutional Networks (GCNs), which use a message-passing paradigm with stacked convolution layers, are foundational methods for learning graph representations. Recent GCN models use various residual connection techniques to alleviate the model degradation problem such as over-smoothing and gradient vanishing. Existing residual connection techniques, however, fail to make extensive use of underlying graph structure as in the graph spectral domain, which is critical for obtaining satisfactory results on heterophilic graphs. In this paper, we introduce ClenshawGCN, a GNN model that employs the Clenshaw Summation Algorithm to enhance the expressiveness of the GCN model. ClenshawGCN equips the standard GCN model with two straightforward residual modules: the adaptive initial residual connection and the negative second-order residual connection. We show that by adding these two residual modules, ClenshawGCN implicitly simulates a polynomial filter under the Chebyshev basis, giving it at least as much expressive power as polynomial spectral GNNs. In addition, we conduct comprehensive experiments to demonstrate the superiority of our model over spatial and spectral GNN models.

==> Clenshaw Graph Neural Networks/www2023/0_abstract.tex <==
\begin{comment}
Graph Convolution Networks (GCNs) are fundamental in graph learning methods, 
which create a paradigm of passing messages on the graph topology within stacked convolution layers. 
Following traditional neural networks, 
residual connections are used in GCNs to alleviate the model degradation problem, 
especially over-smoothing, the most explored cause of degradation. 
However, existing graph residual connections are \textcolor{blue}{either too simple to be expressive 
or too dense to be explainable.} 
Moreover, these works fail to build a connection with deeper characteristics of the graph, 
\textit{i.e. } the spectral aspect of GNNs.

In this paper, we propose Clenshaw Graph Convolution Networks, 
a kind of GCN following the recurrence of the Clenshaw Summation Algorithm. 
In each convolution layer, 
GCN equips Vanilla Graph Convolution with two residual modules: 
the \textit{adaptive initial residual connection} 
and the \textit{negative second-order residual connection} 
(\textit{i.e.} $\mathbf{H}^{(\ell-2)}$ with current layer  $\ell$ ).
We show that by adding this two residual modules, 
ClenshawGNN implicitly 
\textcolor{blue}{\textbf{acts as} a polynomial filter based on(under) the Chebyshev basis \textbf{entangled with non-linear layers}}
\textcolor{red}{(or say: `\textbf{acts like} a polynomial filter based on the Chebyshev basis')}
,
bringing it at least comparable expressive power than polynomial spectral GNNs.  
Extensive experiments demonstrate our model's superiority over spatial and spectral GNN models.    
\end{comment}




Graph Convolutional Networks (GCNs), which use a message-passing paradigm with stacked convolution layers, 
are foundational methods for learning graph representations.
% Graph Convolutional Networks (GCNs), which use the message-passing paradigm with stacked convolution layers, are of foundational importance for learning graph representations. 
{Recent GCN models use various residual connection techniques to alleviate the model degradation problem such as over-smoothing and gradient vanishing.
Existing residual connection techniques, however, fail to 
make extensive use of underlying graph structure as in the graph spectral domain, }
% \textcolor{red}{Recent GCN models use various residual connection techniques to alleviate the model degradation problem, or even leverage residual connections to increase the model's expressive capacity. 
% Existing residual connection techniques, however, fail to
% extensively exploit characteristics 
% from the graph spectral domain,
%  }
which is critical for obtaining satisfactory results on heterophilic graphs.

In this paper, we introduce ClenshawGCN, a GNN model that employs the Clenshaw Summation Algorithm to enhance the expressiveness of the GCN model.
ClenshawGCN equips the standard GCN model with two straightforward residual modules: the \textit{adaptive initial residual connection} and the \textit{negative second-order residual connection}.
We show that by adding these two residual modules, ClenshawGCN implicitly simulates a polynomial filter under the Chebyshev basis, giving it at least as much expressive power as polynomial spectral GNNs.
In addition, we conduct comprehensive experiments to demonstrate the superiority of our model over spatial and spectral GNN models.



% When generating node representations for the next layer(\textit{i.e.} $\mathbf{H}^{(l+1)}$),
% our model should only connect to the initial layer(\textit{i.e.} $\mathbf{H}^{(0)}$) \textit{adaptively},
% and to the {second last layer}(i.e. $\mathbf{H}^{(l-1)}$) \textit{negatively}.
% % The way of $rewiring$ by residual connections
% The construction of 
% this residual connection inherently uses \textbf{Clenshaw Summation Algorithm}, 
% a numerical evaluation algorithm for calculating weighted sums of Chebyshev basis 
% in a \textit{recurrence} way. 

% % The recurring nature of Clenshaw Summation is a good fit with 
% % the layer-wise recurring process of message-passing neural networks. 
% % Such a model is termed Clenshaw Graph Convolutional Network.
% The introduced shortcuts retrofit the graph neural network 
% implicitly as a polynomial filter based on the Chebyshev basis entangle with non-linear layers, bringing it at least comparable expressive power with polynomial spectral GNNs.  
% Experiments demonstrate our model's  superiority 
% either compared with other spatial models with residual connections or with spectral models. 






==> Clenshaw Graph Neural Networks/www2023/1_intro.tex <==
\section{introduction}


% Over the past years, the study and design of neural networks on graph structures have become a popular topic.
The past few years have witnessed the rise of machine learning on graphs, which considers
% implicit or explicit 
relations (edges) between elements (nodes) such as
interactions among molecules \cite{duvenaud2015convolutional, satorras2021n}, 
friendship or hostility between users \cite{fan2019graph, wu2020graph}, and  implicit syntactic or semantic structure in natural language \cite{schlichtkrull2020interpreting, wu2021graph}.

% A paradigm of Graph Neural Networks was 
% proposed in GCN \cite{kipf2016semi},  
% which exploits the underlying graph topology 
% by propagating node features iteratively along the edges. 
% Along with the message-passing steps, 
% information from broader and broader neighborhoods reaches each node. 
GCN~\cite{kipf2016semi} proposed a message-passing paradigm for Graph Neural Networks that exploits the underlying graph topology by propagating node features iteratively along the edges. 
Along with the message-passing steps, each node receives information from growingly expanding neighborhoods.
Such a \textit{propagation} entangled with non-linear \textit{transformation} 
forms a \textit{graph convolution layer} in GCN. 
% denoted as $\mymathhl{f: x \to conv{(x)}}$.

% However, 
% multi-stacked graph convolution layers
% suffer from \textit{model degradation}[][]. 
% Model degradation is the phenomenon 
% when a model's performance come worse with a larger depth.  
% % making it difficult for 
% It hinders neural networks from 
% the benefits of 
% over-parameterization and large inceptions[][]. 

\begin{figure*}[htp]
    \includegraphics[width=1.8\columnwidth]{www2023/pics/residuesV3.png}
    \caption{Illustration of different graph residual connections. \textit{Raw Residue} and \textit{Initial Residue} follows a single-line structure, \textit{Dense Residue} connect densely to all the former layers, while our \textit{Clenshaw Residue} achieves strong expressive power by a neat double-line structure. }
    \label{fig:residues}
    \Description{figure description}
\end{figure*}

Following ResNet \cite{He2016residual}, various GNN models use different residual connection techniques to overcome the problem of \textit{model degradation}. 
As shown in Figure~\ref{fig:residues}, we broadly classify the graph residual connections into three types:




\begin{itemize}[leftmargin = 4mm]
    \item \textbf{Raw Residual Connections} are 
    directly transplanted to GCNs in early attempts \cite{kipf2016semi}, 
    % they connect back to the input $\mymathhl{f: x \to conv{(x)} + x}$ 
    % Early attempts[][] directly transplant 
    % the \textit{raw residual connection} to GCNs, 
    % \textit{i.e.} $\mymathhl{f: x \to conv{(x)}+x}$, 
    but they lose effectiveness when models come deeper\cite{keyulu2018jknet, chen2020gcnii}.   
    % The revelation of the cause  was achieved by
    The reason behind this was gradually
    clarified with the discussion of {\ul \textit{over-smoothing}} \cite{li2018deeper,rong2020dropedge}
    .  
    % \begin{comment}
    % \item  A line of discussion on \textit{over-smoothing} view 
    % GCNs equipped with raw residual connections 
    % as \textit{lazy random walks} 
    % \cite{chen2020gcnii, keyulu2018jknet, wang2019improving}, 
    % which also converge to the \textit{stationary vector}. 
    % Intuited by this,
    % \textbf{initial residual connection} was proposed
    % to simulate \textit{personalized random walks}, instead\cite{klicpera2019appnp, chen2020gcnii}, 
    % and some variants were explored \cite{Liu2021Air,Zhang2022hinder}.
    % However, despite its ability to eliminate over-smoothing, 
    % the initial residual connection is only making a \textit{compromise} 
    % between Laplacian smoothing and keeping identity, 
    % which still follows the \textit{homophily assumption}\cite{mcpherson2001birds}.  
    % % Each smoothed level of node features contributes \textit{positively}  
    % % to the final output.
    % % that is, connected nodes tend to share similar features and labels. 
    % % More extensive use of different fused levels 
    % % is needed for non-homophily graphs[][]. 
    % \end{comment}
    \item  
    \textbf{Initial Residual Connections} \cite{klicpera2019appnp, chen2020gcnii} are intuited by \textit{personalized pagerank}, 
    following the perspective of viewing GCNs with raw residues as \textit{lazy random walk} \cite{keyulu2018jknet, wang2019improving}, 
    which converges to the \textit{stationary vector}. 
    Equipped with initial residues,   
    the final representation implicitly leverages features of all fused levels. 
    % Initial residue at the $\ell$-th layer draws the initial representation closer 
    % to the output by skipping the former $\ell$ convolutions,  
    However, despite its ability to eliminate over-smoothing, 
    % the implicit optimization goal of 
    % seeing from the optimization perspective \cite{Liu2021Air, zhu2021interpreting},
    % initial residual connection is only making a \textit{compromise} 
    % between Laplacian smoothing and keeping identity, 
    % which 
    models with
    initial residual connections in fact employees the \textit{\underline{homophily assumption}} \cite{mcpherson2001birds},  
    that is, the assumption that connected nodes tend to share similar features and labels, 
    which might be unsuitable for heterophilic graphs~\cite{Pei2020GeomGCN, zheng2022hetesurvey}. 
    Some variants are also explored~\cite{Liu2021Air, Zhang2022hinder}, 
    but they still fall into the scope of homophily. 
    % Each smoothed level of node features contributes \textit{positively}  
    % to the final output.
    % that is, connected nodes tend to share similar features and labels. 
    % More extensive use of different fused levels 
    % is needed for non-homophily graphs[][]. 
    \item 
    % There are also \textbf{Denser Residual Connections} [][][]. 
    % Different from {raw residual connection} and {initial residual connection} 
    % that use only \textit{one extra} shortcut for each convolution layer, 
    % these models connect \textit{densely} to all the former layers 
    % at the final step\cite{keyulu2018jknet, chien2021gprgnn} or at each intermediate step\cite{Li2019deep}. 
    There are also \textbf{Dense Residual Connections}, which believe that,    
    by exhibiting feature maps after different times of convolutions and combining them selectively, 
    % for example, by weighted-sum, max-pooling, concatenation, LSTM, \textit{etc}, 
    it is helpful for making extensive use of multi-scale information
    \cite{abu2019mixhop, keyulu2018jknet}.   
    % These works do pull up the limit of expressive power that GNNs may reach.  
    % However, they are not deep in practice, 
    % and it's \underline{\textit{hard to analyze}} what they have actually learned. 
    % Another example is the DenseNet form\cite{iandola2014densenet} tried in \cite{Li2019deep}, 
    % The connection manner in DenseNet \cite{iandola2014densenet} is also exploited by 
    % connecting to all the former layers at each intermediate step~\cite{Li2019deep},  
    % which causes unaffordable space consumption. 
    The connection pattern in DenseNet \cite{iandola2014densenet} is also exploited 
    in ~\cite{Li2019deep}, 
    where they connect each layer to all former layers, incurs unaffordable space consumption.
\end{itemize}

% \begin{figure*}[htp]
%     \label{fig:residues}
%     \includegraphics[width=1.8\columnwidth]{www2023/pics/residuesV3.png}
%     \caption{Illustration of different graph residual connections. \textit{Raw Residue} and \textit{Initial Residue} follows a single-line structure, \textit{Dense Residue} connect densely to all the former layers, while our \textit{Clenshaw Residue} achieves strong expressive power by a neat double-line structure. }
%     \Description{figure description}
% \end{figure*}


% Besides the networks with spatial message-passing dynamics, 
% there is another line of spectral works. 
% The spectral work 
% \begin{comment}[10-12-afternoon]
% \textcolor{blue}{[First way (I prefer this)]}
% On the other hand, 
% the use of multi-scale neighborhoods is closely related to 
% the implementation of \textit{Polynomial Filters} in the \textit{Spectral} GNN domain,   
% where different orders of propagation are combined 
% for effective access to the polynomial terms.
% Spectral GNNs \textcolor{red}{gain its power} 
% from utilizing atomic \textit{components} decomposed from the underlying graph.  
% This \textcolor{red}{motivates} us to inject the characteristics of spectral GNNs 
% into the process of spatial message passing with residual connections. 
% Indeed, 
% existing spectral models like GPRGNN \cite{chien2021gprgnn} already have a sense of `residual connections' 
% in the uses of former information from narrower neighborhoods 
% However, spec models are shallow indeed. 
% In this paper, we concern with GNNs with stacked building blocks entangled with non-linear transformations 
% to benefit from truly deep structures \cite{chen2020gcnii}.


% \textcolor{blue}{[Another way?] On the other hand, 
% the idea of making extensive use of multi-scale neighborhoods is closely related to  
% \textit{Spectral Graph Neural Networks}, 
% which motivates us to {inject the characteristics of spectral GNNs into our model by residual connections}. 
% % (See Section~\ref{sec:poly_filter} for more backgrounds). 
% Different from the spatial message-passing paradigm introduced above,   
% % Spectral GNNs leverage \textit{eigen vectors} of the underlying graph, 
% % which is considered as the set of patterns or components.
% spectral GNNs \textcolor{red}{gain its power} 
% by decomposing the underlying graph into \textit{components}, or atomic \textit{patterns}. 
% Spectral GNNs project features onto these components, 
% and modulate the weights of the components by a \textit{filter}. 
% When this filter is a \textit{polynomial} function on the graph's Laplacian spectrum, 
% explicit decompositions of matrices are avoided, 
% replaced by localized propagations in a finite neighborhood radius. 
% Indeed, 
% existing spectral models like GPRGNN\cite{chien2021gprgnn} have a sense of `residual network' 
% in the uses of former information from narrower neighborhoods. 
% % They differ from spatial residual networks in that,  
% % spectral models are not 
% % built up by the stacking of convolution blocks, 
% % and are not \textit{entangled} with non-linear transformations. 
% However, such models are shallow indeed. 
% In this paper, we concern with GNNs with stacked building blocks entangled with non-linear transformations 
% to benefit from truly deep structures\cite{chen2020gcnii}.
% }
% \end{comment}

\subsubsection*{\ul Residual Connections and Polynomial Filters}
% \header{\bf Residual Connections and Polynomial Filters.}
On the other hand, 
the idea of making extensive use of multi-scale representations is closely related to  
\textit{Spectral Graph Neural Networks}, 
which motivates us to {inject the characteristics of spectral GNNs into our model by residual connections}. 
% (See Section~\ref{sec:poly_filter} for more backgrounds). 
% Different from the spatial message-passing paradigm introduced above,   
% Spectral GNNs leverage \textit{eigen vectors} of the underlying graph, 
% which is considered as the set of patterns or components.
Spectral GNNs {gain their power} 
from utilizing atomic \textit{structural components} decomposed from the underlying graph. 
Spectral GNNs project features onto these components, 
and modulate the importance of the components by a \textit{filter}. 
When this filter is a $K$-order \textit{polynomial} function on the graph's Laplacian spectrum, 
explicit decompositions of matrices are avoided, 
replaced by additions and subtractions of localized propagation results 
within different neighborhood radii, 
building a connection with `residual connection'.

% \begin{comment}
% The expressive power in terms of representing arbitrary polynomial filters has been discussed in 
% former graph residual connection works, especially the dense residual GNNs, 
% for example, MixHop \cite{abu2019mixhop}, 
% where the proof of expressive power is made by setting a tricky case 
% of the transformation matrices. 
% Other than that, GPRGNN \cite{chien2021gprgnn}, 
% which can be viewed as equipped by dense connections at the last layer,
% is also a flexible spectral model.    
% \end{comment}

Often, the problem of polynomial filtering is reduced to 
learning a proper polynomial function in order $K$. 
The expressive power in terms of representing \textbf{arbitrary polynomial filters} has been discussed in 
former graph residual connection works, especially dense residues \cite{abu2019mixhop, chien2021gprgnn}.  
However, 
motivated from the spatial view of message passing, 
these works lose an important part of spectral graph learning: the employee of \textbf{polynomial bases}. 
Polynomial bases are of considerable significance when learning filtering functions.  
Until now, different polynomial bases are utilized, including 
Chebyshev Basis \cite{Defferrard2016cheb, he2022chebii}, 
Bernstein Basis \cite{He2021bern}
etc.\
See the example of Runge Phenomenon in \cite{he2022chebii} for an illustration of its importance.

\subsubsection*{\ul Contributions}
% In conclusion, 
% graph residual connection   
% We are intended to design good graph residual connections. 
This paper focuses on the design of graph residual connections that exploit the expressive power of spectral polynomial filters.
% Until now, though different graph residues are tried, 
% they do not boost graph neural networks as ResNet in computer vision. 
As we have demonstrated, 
% raw residual connections and initial residual connections are limited in \textit{over-smoothing} and 
% \textit{homophily assumption}, respectively. 
raw residual connections and initial residual connections are primarily concerned with mitigating \textit{over-smoothing}, and they commonly rely on the \textit{homophily assumption}.
% Some dense residual connections do bring up the expressive 
% power a GNN might reach,
% with analyses aligning the spatial process with  \textit{potentially arbitrary} spectral polynomial filter. 
% However, the importance of polynomial bases is neglected.
Some dense residual connections do increase the expressive capacity of a GNN, with analyses aligning the spatial process with a potentially arbitrary spectral polynomial filter.
Unfortunately, these works do not take the significance of different polynomial bases into account and are therefore incapable of learning a more effective spectral node representation.

In this paper, we introduce ClenshawGCN, a GNN model that
employs the Clenshaw Summation Algorithm to {enhance the expressiveness of the GCN model}. 
More specifically, we list our contributions as follows:
\begin{itemize}[leftmargin=4mm]
    \item \textbf{Powerful residual connection submodules}. We propose ClenshawGCN, a message-passing GNN which borrows spectral power by adding two simple residual connection modules to each convolution layer: 
    an \textit{adaptive initial residue} and a \textit{negative second order residue}; 
    \item \textbf{Expressive power in terms of polynomial filters} We show that a $K$-order ClenshawGCN simulates \textit{any} $K$-order polynomial function based on the \textit{Chebyshev basis of the Second Kind}. 
    More specifically, 
    the \textit{adaptive initial residue} allows for 
    the flexibility of coefficients,
    % representing any polynomial filters
    while the \textit{negative second order residue} allows for the implicit use of 
    Chebyshev basis. We prove this by the Clenshaw Summation Algorithm for Chebyshev basis (the Second Kind). 
    \item \textbf{Outstanding performances}. We compare ClenshawGCN with both spatial and spectral models.  
    Extensive empirical studies demonstrate that ClenshawGCN outperforms 
    both spatial and spectral models on various datasets.
\end{itemize}



% % We propose a model that is both \textit{expressive} and \textit{neat}.  
% For expressiveness, our model implicitly mimics a polynomial filter, 
% where residual connections serve as a bridge between spectral and spatial characteristics.
% For simplicity, our model only adds \textit{two} shortcuts to each convolutional block,  
% and it keeps the same recurrence form for each layer, 
% with maximum retention of the vanilla convolutions. 



==> Clenshaw Graph Neural Networks/www2023/1_intro_old.tex <==
\section{introduction}

\begin{figure}[htp]
\includegraphics[width=1.\columnwidth]{www2023/pics/residues.png}
\caption{figure caption}
\Description{figure description}
\end{figure}

% Over the past years, the study and design of neural networks on graph structures have become a popular topic.
The past few years have witnessed the rise of the graph learning field. 
In the graph learning field, 
% implicit or explicit 
relations (edges) between elements (nodes) are considered, 
\textit{e.g.} interactions among molecules[][], 
friendship or hostility between users[][],  
implicit syntactic or semantic structure in natural language[][]
and so on.
A paradigm of Graph Neural Networks was 
proposed in GCN\cite{kipf2016semi},  
% as an extreme simplification of 
which exploits the underlying graph topology 
by propagating node features iteratively along the edges. 
Along with the passing steps, 
information from a broader neighborhood is reached for each node. 
Such a \textit{propagation} entangled with non-linear \textit{transformation} 
forms a \textit{graph convolution layer} in GCN, 
denoted as $\mymathhl{f: x \to conv{(x)}}$.

However, just like what Convolution Neural Networks (CNNs) 
were faced with during its development[][], 
% GCN stacked by multiple convolution layers 
multi-stacked graph convolution layers
suffer from 
\textit{model degradation}[][]. 
Model degradation is the phenomenon 
when a model's performance come worse with a larger depth.  
% making it difficult for 
It hinders neural networks from 
the benefits of 
over-parameterization and large inceptions[][]. 


Model degradation of CNNs was solved by ResNet in the year of 2016\cite{He2016residual}.
% when He \textit{et. al.} raised \textit{residual connection}. 
This milestone module boosts CNNs in an extremely simple way: 
it only \textit{wraps} each convolution block with the $input$, 
denoted as $\mymathhl{f: x \to conv{(x) + x}}$
\footnote{Here, \textit{conv} is the convolution layer in CNN.}.


\textcolor{red}{[Recent works \& Perspective $\to$ Spectral Model]}\\
  
\begin{comment}
Following ResNet, 
researchers try to apply different residual connections  
to GCN[][][][][][][].
    \item \textbf{Raw Residual Connection}. 
    Early attempts[][] directly transplant 
    the \textit{raw residual connection} to GCNs, 
    % \textit{i.e.} $\mymathhl{f: x \to conv{(x)}+x}$, 
    but it doesn't work.   
    % The revelation of the cause  was achieved by
    The reason behind was gradually
    clarified with the discussion of \textit{over-smoothing}[][][]. 
    % Oversmoothing is the most discussed reason for the degradation of
    % GCNs, meaning that with features would be ...
    \item \textbf{Initial Residual Connection}. Along with the understanding of over-smoothing, \textit{initial residual connection} was proposed[] and explored with some variants[][]. However, despite of its ability to eliminate over-smoothing, 
    initial residual connection is only making a \textit{compromise} 
    between Laplacian smoothing and keeping identity, 
    which still follows the \textit{homophily assumption}[], 
    where each smoothed level of node features contributes \textit{positively}  
    to the final output.
    % that is, connected nodes tend to share similar features and labels. 
    More extensive use of different fused levels 
    is needed for non-homophily graphs[][]. 
    \item \textbf{Dense Residual Connections.} 
\end{comment}

Following ResNet, 
researchers try to apply different residual connections  
to GCN[][][][][][][].
Early attempts[][] directly transplant 
the \textit{raw residual connection} to GCNs, 
% \textit{i.e.} $\mymathhl{f: x \to conv{(x)}+x}$, 
but it doesn't work.   
% The revelation of the cause  was achieved by
The reason behind was gradually
clarified with the discussion of \textit{over-smoothing}[][][]. 

Along with the understanding of over-smoothing, 
\textit{initial residual connection} was proposed[] and explored with some variants[][]. 
% which can be roughly expressed as 
% $\mymathhl{f: x \to \alpha conv{(x) + \beta x^{*}}}$, 
% where $x^{*}$ is the initial representation of the node, 
% and $\alpha$ and $\beta$ are fixed[][] or not fixed. 
However, despite its ability to eliminate over-smoothing, 
initial residual connection is only making a \textit{compromise} 
between Laplacian smoothing and keeping identity, 
which still follows the \textit{homophily assumption}[], 
where each smoothed level of node features contributes \textit{positively}  
to the final output.
% that is, connected nodes tend to share similar features and labels. 
% It has been More extensive use of different fused levels 
% is needed for non-homophily graphs[][].  
Here comes our first motivation:
\begin{tcolorbox}[boxrule=0.pt,height=15mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\textbf{Motivation I}: Making flexible use of different 
fused levels of representations. 
\end{tcolorbox}
% \end{comment}

There are also \textit{denser residual connections} [][][]. 
Different from raw residual connection and initial residual connection 
that use \textit{only one} extra shortcut for each convolution layer, 
these models connect densely to the \textit{all} the former layers 
at the final step[] or at each intermediate step[][]. 
Some of these works do pull up the limit of expressive power that GNNs may reach[][], 
but their real actions are hard to analyze, 
and are often not very deep in use[][].

\begin{tcolorbox}[boxrule=0.pt,height=15mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\textbf{Motivation II}: 
Constructing \textbf{neat} residual connections 
for easier analysis. 
\end{tcolorbox}

Though limited by the underlying homophily assumption, 
the progress made by initial residual connection 
gives a hint of making more use of graph topology. 
Over-smoothing is a GNN-specific cause of degradation.  







\textcolor{red}{[Our Model]}



When designing specific components, graph neural networks(GNNs) and general neural networks have both similar and special concerns. \textit{Residual connection}, what we are concerned about in this work, is such a component. 
Residual connection was first raised in ResNet\cite{He2016residual} to stack deep CNNs. 
It is famous for significant simplicity and strong ability in solving the \textit{model degradation} problem. 

On the other hand, there are causes of model degradation on the graph that are related to the topology of the graph, such as over-smoothing, which is different from the traditional model; 
in the work to be presented today, by constructing shortcuts, we can even bridge the connection between changing the path of information flow process and the graph Fourier and graph polynomial filters.



\\
\begin{comment}
    \textcolor{red}{[TODO: make the related work part more precise]}
\subsubsection*{\textbm{Residual Connections in Graph Learning}}
In the current literature, the following types of Residual Connection can be found: 
(1) one-hop to the previous layer; 
(2) one-hop to the initial layer; 
(3) densely connected to all the previous layers.

\subsubsection*{\underline{Residual Connection to the Previous Layer}}

In Vanilla GCN, each layer of convolution can be seen as a propagate of information on the graph.
This problem is known as oversmoothing, and is one of the more explored causes of GNN model degradation.
Vanilla GCN tries to connect to the Residual Connection of the previous layer, but the oversmoothing problem is still not solved: from the wandering point of view, connecting back to the Raw Residual Connection of the previous layer with $\alpha$.
is equivalent to turning a random walk into a lazy random walk.
The lazy random walk converges to the steady state (assuming the graph is connected and not bipartite), which corresponds to the principal eigenvector of the adjacency matrix.

\subsubsection*{\underline{Residual Connection to the Initial Layer}}

To alleviate the oversmoothing problem, the initial residual connection is connected back to the representation of the initial layer with a certain probability at each layer.
That is, the representation of the next layer is derived from the initial representation with a certain probability, instead of the neighborhood messages after multiple confusions.
This tilts a node's tendency towards maintaining its own feature against being over-smoothed.

It is noted in [] that initial Residual can be viewed as solving such an optimization problem: ( )(1).
The trade-off between multi-hop neighborhood information and initial features can also be seen in it.

In addition, there are variants of the Initial Residual Connection
AirGNN (GLASSO) takes a nodewise, sub-node form of $\alpha$ selection, but the essence of the solution is to use the Elastic Likelihood (ELL) method.
However, its essence is to solve the optimization problem improved by Elastic Lasso (1).
The object of its solution is still the homophiliy assumption.

Wentao Zhang et al. decoupled the Transformation and Propagation layers in the Convolution layer and adopted the Initial Residual Connection respectively, which is considered to solve the model degradation and over-smoothing problems, respectively.
The connection coefficients of Initial Residual are learned from the concatenation of the current layer and the initial layer.
However, it is still mainly applicable to homogeneous maps.

% Densely Forward Connected Residual Connection
\subsubsection*{\underline{Densely Connected Residual Connection
}}


Raw Residual Connection and Initial Residual Connection
both use some kind of single-line structure.
Some work suggests that displaying multiple representations of intermediate layers (i.e., feature maps for each level of confusion) simultaneously, 
and then selectively combining them with summation, max-pooling, concatenation, lstm, etc., to exploit more valid information (JKNet, MixHop). Theoretically, these works do pull up the upper limit of the expressive power that GNNs may reach, but these models are not very deep in use, and what is actually learned is not clear.

As another example, Li2019 tried a form of dense connectivity in DenseNet, but the space consumption associated with such connectivity is unaffordable.

In addition, work on polynomial filters on individual graphs also utilizes information from all intermediate layers in their implementation, including GPRGNN, ChebyNet, BernNet, etc. These works perform well on heterogeneous graphs, but formally, they differ significantly from Residual: they appear to be staked, whereas a work like ResNet is more like having a forward line with a more consistent iterative form.

\end{comment}


\subsubsection*{\textbf{Our Model}}

We introduced a new Residual Connection, which, unlike single-line connections and dense connections, has a two-line structure: the initial residual is simply a shortcuts to the upper layer, a change that keeps the structure of the model simple, but brings a Boost effect.

Why does this connection work so well?
First, it no longer follows the assumption of homogeneity, a consideration similar to that of GPRGNN, and what's more, its wiring (construction/rewiring) implicitly exploits the recursive relationship between Chebyshev bases, allowing for a more thorough exploitation of the layers - yes, just by a negative second shortcut. - The general idea behind this construction comes from a method that recursively evaluates the summation of polynomial bases: the Clenshaw algorithm.
This will be explained in detail in a later section. And we performed an ablation study to verify the effect of these two components.


\subsubsection*{\textbf{Deep or linear?}}

When ignoring linear transformation and activation together with propagation entangle, the model becomes a model on the spectral domain (linear GNN). However, we still choose an entangle together in such a way that it becomes a true `deep' model.

% Translated with www.DeepL.com/Translator (free version)


\newpage


==> Clenshaw Graph Neural Networks/www2023/2_Preliminaries.tex <==
\section{Preliminaries}
\subsection{Notations}
% \textcolor{blue}{[Graph]}\\
% \subsubsection*{\ul Notations for a Graph}
We consider a simple graph $\mathcal{G}=(\mathcal{V}, \mathcal{E}, \mathbf{A})$, 
% a simple graph $\mathcal{G}$ with 
where $\mathcal{V} = \{1, 2, \cdots, n \}$ is a finite node-set with $|\mathcal{V}|=n$, 
$\mathcal{E}$ is an edge-set with  $|\mathcal{E}|=m$,
and $\mathbf{A}$ is an unnormalized adjacency matrix.
$\mathcal{L} = \mathbf{D} - \mathbf{A}$ denotes $\mathcal{G}'s$ unnormalized graph Laplacian,
where $\mathbf{D}=\text{diag}\{d_{1}, \cdots, d_{n}\}$
is the degree matrix with $d_i = \sum_{j}{\mathbf{A}_{ij}}$. 
% Denote $\|\mathcal{V}\|=n$, $\|\mathcal{E}\|=m$.

Following GCN, we add a self-connecting edge is to each node,
and conduct symmetric normalization on $\mathcal{L}$ and $\mathbf{A}$.
The resulted \textit{self-looped symmetric-normalized} 
adjacency matrix and Laplacian are denoted as 
$\tilde{\mathbf{P}} = (\mathbf{D}+\mathbf{I})^{-1/2} (\mathbf{A}+\mathbf{I}) (\mathbf{D}+\mathbf{I})^{-1/2}$ and $\tilde{\mathcal{L}}
= \mathbf{I} - \tilde{\mathbf{P}}
$, respectively. 

% \subsubsection*{\ul Notations for Node Classification Task}
% \comment{
% Further, we consider a node classification problem setting where each node has an $f$-dimensional feature and is labeled as one of $c$ classes. 
% The features and one-hot labels of $\mathcal{V}$ are denoted as 
% $\mathbf{X} \in \mathbb{R}^{n \times f}$ and  
% $\mathbf{Y} \in \mathbb{R}^{n \times c}$, respectively, 
% with the $i$-th row of the matrices corresponding to the feature and label of node $i$. 
% Only a subset of $ \mathcal{V}$are given labels, 
% denoted as $\mathcal{V}_c$, 
% and the unlabeled node set is denoted as $\mathcal{V}_u$, 
% their corresponding labels are  $\mathbf{Y}_c$ and $\mathbf{Y}_u$. 
% The goal of Graph Neural Networks(GNNs) is 
% to map $\mathbf{X}$ to $\hat{\mathbf{Y}}\in \mathbb{R}^{n \times c}$, 
% making $\hat{\mathbf{Y}}_u$  a good prediction of unknown labels $\mathbf{Y}_u$.
% }

Further, we attach each node with an $f$-dimensional raw feature and denote the feature matrix as $\mathbf{X} \in \mathbb{R}^{n \times f}$. 
Based on the the topology of underlying graph, 
GNNs enhance the raw node features to better representations for downstream tasks, 
such as node classification or link prediction.

\subsection{Spatial Background}
\subsubsection*{\ul Layer-wise Message Passing Architecture}
From a spatial view, 
the main body of a Graph Neural Network is a stack of \textit{convolution} layers, 
who broadcast and aggregate feature information along the edges. 
Such a graph neural network is also called a Message Passing Neural Network (MPNN).
To be concrete, 
we consider an MPNN with $K$ graph convolution layers 
and denote the nodes' representations of the $\ell$-th layer as $\mathbf{H}^{(\ell)}$. 
$\mathbf{H}^{(\ell)}$ is constructed 
based on $\mathbf{H}^{(\ell-1)}$
by an \textit{propagation} and  possibly a \textit{transformation} operation. 
For example, in Vanilla GCN~\cite{kipf2016semi}, 
the convolution layer is defined as 
\begin{align}
    \label{eq:gcn_conv}
    \mathbf{H}^{(\ell)} = \sigma( \tilde{\mathbf{P}}\mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)}) ),
\end{align}
whose $propagation$ operator is $\mymathhl{f: {\mathbf{H}}^{(\ell-1)} \to \tilde{\mathbf{P}}\mathbf{H}^{(\ell-1)}}$ 
and \textit{transformation} operator is $\mymathhl{f: \tilde{\mathbf{P}}\mathbf{H}^{(\ell-1)} \to 
\sigma( \tilde{\mathbf{P}}\mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)}) )}$. 

% For specific denotation,  
Extra transformations, or probably combinations,  
are applied before and after the stack of 
$K$ convolution layers 
to form a map from  $\mathbf{X}$ to the {final output} $\hat{\mathbf{Y}}$, 
which is determined by the downstream task, 
% For example, 
% to the initial features and final predictions,
\textit{e.g.} 
$\mathbf{H}^{(0)}=\text{MLP}(\mathbf{X}; \mathbf{W}^{(0)})$ 
and $\hat{\mathbf{Y}}=\text{SoftMax}(\text{MLP}(\mathbf{H}^{(K)}; \mathbf{W}^{(K+1)}))$ 
for node classification tasks. 
In this paper, a slight difference in notation lies in that, 
we denote the input of convolution layers to be  $\mathbf{H}^{*}$, instead of $\mathbf{H}^{(0)}$,  
and introduce notations $\mathbf{H}^{(-1)}$ and $\mathbf{H}^{(-2)}$ as zero matrices
for simplicity of later representation.

% \subsubsection*{\textcolor{red}{\underline{Use of Residual Connections}}}

\subsubsection*{\ul Entangled and Disentangled Architectures}
% \textcolor{blue}{(This paragraph can be deleted later.)}
% \textcolor{red}{Obviously (change a word)}, 
The motivations for \textit{propagation} and \textit{transformation} 
in a convolution layer differ. 
\textit{Propagations} are related to
% the spread of influence on 
graph topology, 
analyzed as an analog of 
walks~\cite{keyulu2018jknet, wang2019improving, klicpera2019appnp, chen2020gcnii}, 
diffusion processes~\cite{zhao2021adaptive, klicpera2019diffusion, chamberlain2021grand}, 
% polynomials~\cite{Wu2019sgc, chen2020gcnii}, 
etc.\ , 
while the 
\textit{entangling} of \textit{transformations} between \textit{propagations} 
follows behind the convention of deep learning. 
A GNN is classified under a disentangled architecture 
if the \textit{transformations} are disentangled from \textit{propagations}, such as APPNP~\cite{klicpera2019appnp} and GPRGNN~\cite{chien2021gprgnn}. 
Though it is raised in ~\cite{Zhang2022hinder} that 
the entangled architecture tends to cause model degradations, 
we observe that GCNII~\cite{chen2020gcnii} under the entangled architecture does not suffer from this problem. 
% [TODO: Add some counter states in deep GNNs.]
So we follow the use of entangled transformations as in Vanilla GCN, 
and leverage the identity mapping of weight matrices as in GCNII.



\subsection{Spectral Background}
% \textcolor{blue}{[Graph Fourier Transformation, Graph signal Filtering, Localized polynomial filters]} 
\subsubsection*{\ul Spectral Definition of Convolution}
% $\mathbf{x}$ (Graph signal)
% From a spectral view, the geometric structure of the underlying graph is accounted for another way. 
Graph spectral domain leverages the geometric structure of underlying graphs in another way~\cite{Shuman2013}.

Conduct eigen-decomposition on $\tilde{\mathcal{L}}$, 
i.e. $\tilde{\mathcal{L}} = \mathbf{U} \mathbf{\Lambda} \mathbf{U}^T$, 
% $\mathbf{\Lambda} = \text{diag} \{ \lambda_1, \lambda_2, \cdots, \lambda_n \}$
the spectrum $\mathbf{\Lambda}$  
$= \text{diag} \{ \lambda_1, \cdots, \lambda_n \} $ 
is in non-decreasing order.  
% Correspondingly, the eigendecomposition of $\tilde{\mathbf{P}}$ is 
% $\mathbf{U} \mathbf{\Lambda} \mathbf{U}^T$
% where $ \mathbf{\Lambda} = \mathbf{I} -  \mathbf{\Gamma}$.
Since $\tilde{\mathcal{L}}$ is real-symmetric, 
elements in $\mathbf{\Lambda}$ 
% and $\mathbf{\Lambda}$ 
are real, 
and $\mathbf{U}$ is a complete set of $n$ orthonormal eigenvectors, 
% Conduct eigendecomposition on $\tilde{\mathbf{P}}$
% \footnote{
% is 
% }
% , 
% i.e. 
% % $\tilde{\mathcal{L}} = \mathbf{U} \mathbf{\Gamma} \mathbf{U}^T$.
% % Correspondingly, the eigendecomposition of $\tilde{\mathbf{P}}$ is 
% $\tilde{\mathbf{P}} = \mathbf{U} \mathbf{\Lambda} \mathbf{U}^T$
% % where $ \mathbf{\Lambda} = \mathbf{I} -  \mathbf{\Gamma}$.
% since $\mathcal{L}$ is real-symmetric, 
% elements in $\mathbf{\Gamma}$ and $\mathbf{\Lambda}$ are real, 
% and $\mathbf{U}$ is a complete set of $n$ orthonormal eigenvectors, 
% denoted as $\{\mathbf{u}_i\}_{i=1,2,\cdots,n}$, or $\mathbf{U}$ as a whole. 
% As an analogy to \textit{classic Fourier transform}, 
% $\{\mathbf{u}_i\}$
which is used as a basis of \textit{frequency components} 
analogously to \textit{classic Fourier transform}
. 

Now consider a column in $\mathbf{X}$ as a \textit{graph signal} 
scattered on $\mathcal{V}$, 
denoted as $\mathbf{x} \in \mathbb{R}^{n}$. 
% we can project $\mathbf{x}$ on the 
% the \textit{graph Fourier transform} projects $\mathbf{x}$ onto $\mathbf{U}$ 
% the \textit{responses} of all the \textit{frequency components} are calculated 
\textit{Graph Fourier transform} is defined as 
$\mymathhl{\hat{\mathbf{x}} := \langle \mathbf{U}, \mathbf{x}\rangle = \mathbf{U^T x}}$, 
which projects graph signal $\mathbf{x}$ to the \textit{frequency responses}  of basis components  $\hat{\mathbf{x}}$. 
It is then followed by {\textit{{modulation}}}, 
which can be presented as
$\mymathhl{\mathbf{\hat{x}}^{*}:= g_{\mathbf{\theta}}\mathbf{\hat{x}} = \text{diag}\{\theta_1, \cdots \theta_n \} \mathbf{\hat{x}}} $. 
% where $g_{\mathbf{\theta}}$ can be represented as  $\text{diag}\{\theta_1, \cdots \theta_n \}$, 
After modulation, 
$\textit{inverse Fourier transform}$: $\mymathhl{\mathbf{x}^{*}:= \mathbf{U}\mathbf{{\hat{x}}^{*}}}$
transform $ \mathbf{{\hat{x}}^{*}} $ back to the spatial domain.
The three operations form a spectral definition of \textit{convolution}:
\begin{align}
    \label{eq:graph_fourier}
    g_{\theta} \star \mathbf{x} = \mathbf{U}g_{\theta}\mathbf{U}^T\mathbf{x}, 
\end{align}
which is also called \textit{spectral filtering}. 
Specifically, when $\theta_i = 1-\lambda_i$, 
$\mathbf{U}g_{\theta}\mathbf{U}^T\mathbf{x} \equiv \tilde{\mathbf{P}}\mathbf{x}$, 
giving an spectral explanation of GCN's convolution in Equation~\eqref{eq:gcn_conv}.


\subsubsection*{\ul Polynomial Filtering}
\label{sec:poly_filter}
% In \eqref{eq:graph_fourier}, 
% The filtering function $g_{\theta$ modulates each frequency response in $\mathbf{\hat{x}}$ to a rescaled one. 
% $g_{\mathbf{\theta}}$ can be parameterized as  $\text{diag}\{\theta_1, \cdots \theta_n \}$, 
% where $\theta_i$ is the rescaling coefficient of 
% $\mathbf{x}$'s frequency response on the $i$-th component.  
% Then Equation\eqref{eq:graph_fourier} becomes
% \begin{align}
    % \label{eq:graph_fourier_2}
    % g_{\theta} \star \mathbf{x} = \mathbf{U}  \text{diag}\{\theta_1, \cdots \theta_n \} \mathbf{U}^T\mathbf{x}.
% \end{align}
The calculation of $\mathbf{U}$ in Equation~\eqref{eq:graph_fourier} is of prohibitively expensive. 
% However, \eqref{eq:graph_fourier_2} demands explict eigendecomposition. 
To avoid explict eigen-decomposition of 
${\mathbf{U}}$, 
$g_{\theta}$ is often defined as a polynomial function of a frequency component's corresponding eigenvalue parameterized by $\theta$, 
that is, 
$$
\mathbf{{\hat{x}}^{*}}_i = g_{\theta}(\lambda_i)\langle \mathbf{U}_i, \mathbf{x} \rangle.
$$
The spectral filtering process then becomes
% $$
% \mathbf{U}g(\mathbf{\Lambda})\mathbf{U}^T\mathbf{x}
% $$
\begin{align}
    \label{eq:poly_filter}
    g_{\theta} \star \mathbf{x} = \mathbf{U}g_{\theta}(\mathbf{\Lambda})\mathbf{U}^T\mathbf{x} 
                \equiv  g_{\theta}(\tilde{\mathcal{L}})\mathbf{x}, 
\end{align}
% , which equals $g(\tilde{\mathcal{L}})\mathbf{x} $. 
where $g_{\theta}(\tilde{\mathcal{L}})\mathbf{x}$ elimates eigen-decomposition 
and can be calculated in a localized way in $\mathcal{O}(|\mathcal{E}|)$
~\cite{Defferrard2016cheb, kipf2016semi}. 


\begin{tcolorbox}[boxrule=0.2pt,height=30mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\begin{definition}[Polynomial Filters]
    \label{def:Polynomial Filters}
    Consider a graph whose Laplacian matrix is $\mathcal{\tilde{L}}$ and 
    % whose eigen-decompsition is 
    % $\mathcal{\tilde{L}} = \mathbf{U}\mathbf{\Lambda}\mathbf{U}^T$, 
    use the set of orthonormal eigenvectors of $\mathcal{\tilde{L}}$ 
    as the frequency basis, 
    % with coresponding eigenvalues $ \left\{  \right\}$
    % consider a signal $x$ on this graph and take $U$ as the frequency basis, 
    a \textbf{polynomial filter} is a process that scales each frequency component of the input signal by $\mymathhl{g_{\theta}(\lambda)}$, 
    where $g_{\theta}$ is a polynomial function and $\lambda$ is the corresponding 
    eigenvalue of the frequency component.
\end{definition}
\end{tcolorbox}

% \textcolor{blue}{Equivalently}
Equivalently, we can define the filtering function on 
the spectrum of $\mathbf{\tilde{P}}$, instead of $\tilde{\mathcal{L}}$. 
Since $\mathbf{\tilde{P}} = \mathbf{I} - \tilde{\mathcal{L}}$, $\mathbf{\tilde{P}}$ and $\tilde{\mathcal{L}}$ share the same set of orthonormal eigenvectors $\mathbf{U}$, 
and the spectrum of  $\mathbf{\tilde{P}}$, denoted as $\mathbf{M} = \{ \mu_1, \cdots, \mu_n\}$, satisfies 
$\mu_i = 1- \lambda_i (i=1,\cdots, n)$ . 
Thus, the filtering function can be defined as $h_{\theta}$, 
where 
\begin{equation}
    \label{eq:poly_filter_definition}
    \mymathhl{h_{\theta}(\mu) \equiv g_{\theta}(1-\mu)}.
\end{equation}
% $$\mymathhl{b_{\theta}(\mu) \equiv g_{\theta}(1-\lambda)}$$. 
In Section~\ref{sec:method}, 
for the brevity of presentation, 
we will use this equivalent definition.



% followed by $\mymathhl{\textit{modulation}}$

% Suppose that the eigenvectors are in an ascending order with respect to their corresponding eigenvalues, 
% denoted as $0 \leq \lambda_1 \leq \lambda_2 \leq \cdots < \lambda_n$. 
% Consider $\{u_i\}_i$ as signals scattered on the graph,  
% the smaller $\lambda_i$ is, the smoother $u_i$ would be. 
% So, $\{u_i\}_i$ is used as an analog of Fourier frequency components. 

% The graph Fourier
% The table below summaries the terms in graph Fourier transform 
% analogously with the classic Fourier transform: 

% In analogy with classical Fourier transform, i.e. $\hat{f}(\xi)=\langle \rangle$




\subsection{Polynomial Approximation and Chebyshev Polynomials}
\subsubsection*{\ul Polynomial Approximation}
Following 
the idea of polynomial filtering (Equation~\eqref{eq:poly_filter}), 
the problem 
% of the spectral graph domain 
then becomes the approximation of polynomial $g_{\theta}$. 
A line of work approximates $g_{\theta}$ by 
% a polynomial $h$ of lower order 
% based on 
some truncated polynomial basis $\{\phi_i(x)\}_{i=0}^{i=K}$
up to the $K$-th order, 
\textit{i.e.}  
$$
    g_{\theta}(x) = \sum_{k=0}^{K} \theta_i \phi_i(x),
$$
where
$\vec{\theta} = \left[ \theta_0, \cdots, \theta_K \right]\in \mathbb{R}^{K+1}$ is the coefficients.   
In the field of polynomial filtering and spectral GNNs, 
different bases have been explored for $\{\phi_i(x)\}_{i=0}^{i=K}$, 
including Chebyshev basis~\cite{Defferrard2016cheb}, 
Bernstein basis~\cite{He2021bern}, 
Jacobi basis~\cite{Wang2022jacovi}, {etc}.

\subsubsection*{\ul Chebyshev Polynomials}
Chebyshev basis has been explored since early attempts for the approximation of $g_{\theta}$~\cite{Defferrard2016cheb}. 
Besides Chebyshev polynomials of the first kind ( $\{T_i(x)\}_{i=0}^{\infty}$ ), 
the second kind ( $\{U_i(x)\}_{i=0}^{\infty}$ ) is also wildly used. 

Both $\{T_i(x)\}_{i=0}^{\infty}$ and $\{U_i(x)\}_{i=0}^{\infty}$ 
can be generated by a \textit{recurrence relation}: 
\begin{align}
        \label{eq:Urec}
        &T_{0}(x)  = 1, \quad
        T_{1}(x)  = x, \nonumber \\ 
        % &\cdots, 
        &T_{n}(x) = 2xT_{n-1}(x) - T_{n-2}(x). \quad(n=2, 3, \cdots)  
        \nonumber  \\ \nonumber \\
        &U_{-1}(x)  = 0, \quad
        U_{0}(x) = 1, 
        U_{1}(x)  = 2x,\nonumber   \\
        % &\cdots,
        &U_{n}(x) = 2xU_{n-1}(x) - U_{n-2}(x). \quad(n=1, 2, \cdots)
\end{align}

% \begin{tcolorbox}[boxrule=0.2pt,height=33mm,boxrule=0.pt,colback=blue!2!white]
% % \begin{definition}[Chebyshev Polynomials (First Kind)]
% \begin{corollary}[Recurrence Relation for the First-kind Chebyshev polynomials]
%     For the Chebyshev polynomials $\left\{T_n(x)\right\}$ of the first kind, 
%     \begin{align*}
%         T_{0}(x)  &= 1, \quad
%         T_{1}(x) = x, \\
%         &\cdots, \\
%         T_{n}(x) &= 2xT_{n-1}(x) - T_{n-2}(x) \quad(n=2, 3, \cdots) 
%         % &\cdots.
%         % \\&\quad\quad\quad\quad(i=2, 3, \cdots)
%     \end{align*}
% \end{corollary}
% \end{tcolorbox}


% \begin{tcolorbox}[boxrule=0.2pt,height=38mm,boxrule=0.pt,colback=blue!2!white]
% \begin{corollary}[Recurrence Relation for the Second-kind Chebyshev polynomials]
%     The first Chebyshev Polynomials $\left\{U_n(x)\right\}$  of the second kind,   
%     \begin{align*}
%             U_{-1}(x)  &= 0, \quad
%             U_{0}(x) = 1, \quad
%             U_{1}(x)  = 2x, \\
%             &\cdots,\\
%             U_{n}(x) &= 2xU_{n-1}(x) - U_{n-2}(x)\quad(n=1, 2, 3, \cdots)
%     \end{align*}
% \end{corollary}
% \end{tcolorbox}

The recurrence relation is used in ChebyNet~\cite{Defferrard2016cheb} 
for accelarating the computing of polynomial filtering.
Note that we start the second kind from $U_{-1}$, which will be used in later proof in Section~\ref{sec:neg_residue}.


\subsection{Residual Network Structures}
% \textcolor{blue}{[TODO: (1)list some model structures that would be used later; (2)mention recent works of `difference residuals']}
We have discussed some graph residual connections in Introduction . 
In this section, we list some model in detail for illustration of residual connections.
\begin{comment}
{
% \subsubsection*{Initial Residues.}
% \begin{itemize}[leftmargin = 4mm]
    % \item 
The \textbf{initial residual connection} is connected back to the representation of the initial layer with a \textit{fixed} probability at each layer. 
\textbf{APPNP}~\cite{klicpera2019appnp} is the convolution of 
$$
    \mathbf{H^{(\ell+1)}} = (1-\alpha) \tilde{\mathbf{P}}\mathbf{H^{(\ell)}} 
        + \alpha \mathbf{H^{*}}, 
$$
which iteratively solves the optimization problem:
$$
    \underset{\mathbf{H} \in \mathbb{R}^{n \times d}}{\arg \min } \mathcal{L}_2(\mathbf{H}):=\frac{\alpha}{2(1-\alpha)}\left\|\mathbf{H}-\mathbf{H}^{*}\right\|_F^2+\frac{1}{2} \operatorname{tr}\left(\mathbf{H}^{\top} \tilde{\mathcal{L}} \mathbf{H}\right). 
$$
The optimization goal reveals the underlying 
\textit{homophily assumption}, 
% Seeing from the optimization goal, 
where initial residual connection is only making a \textit{compromise} 
between Laplacian smoothing and keeping identity. 
}
\end{comment}


\textbf{GCNII} 
% can be seen as a \textit{deep} version of APPNP 
% in entangling non-linearity in convolutions. GCNII 
equips 
the vanilla GCN convolution with two techniques: initial residue and identity mapping:   
% and succeed in building deep models
% GCNII's convolution layer is 
\begin{equation}
        \label{eqn:gcnii_analysis}
        \hspace{-0.7mm} \mathbf{H}^{(\ell)} \hspace{-0.7mm}= \hspace{-0.7mm}
      \sigma  \hspace{-0.7mm}\left(  \hspace{-0.7mm}\left( \hspace{-0.5mm}  (1  \hspace{-0.7mm}-  \hspace{-0.7mm}\alpha)\tilde{\mathbf{P}}
            \mathbf{H}^{(\ell-1)}  \hspace{-0.7mm} +  \hspace{-0.7mm}
            \alpha\mathbf{H}^{*}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}
          \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
            \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right).
        \end{equation}

Ignoring non-linear transformation, GCNII 
iteratively solves the optimization problem:
\begin{equation}
    \label{eq:opt_initial}
    \underset{\mathbf{H}}{\arg \min} \quad  
    % \mathcal{L}_2(\mathbf{H}):=
    {\alpha}\left\|\mathbf{H}-\mathbf{H}^{*}\right\|_F^2+ (1-\alpha) \operatorname{tr}\left(\mathbf{H}^{\top} \tilde{\mathcal{L}} \mathbf{H}\right).   
\end{equation}
  

The optimization goal reveals the underlying 
\textit{homophily assumption}, 
% Seeing from the optimization goal, 
where initial residual connection is only making a \textit{compromise} 
between Laplacian smoothing and keeping identity. 

    
\textbf{AirGNN}~\cite{Liu2021Air} proposes an extension for initial residue, 
% where the initial residue is
where the first term of optimization problem in Equation~\eqref{eq:opt_initial} 
is replaced by the $\ell_{21}$ norm. 
By solving the optimization problem, AirGNN adaptively choose $\alpha$. 
However, limited by the optimization goal, 
AirGNN still falls into the homophility assumption. 

\textbf{JKNet}~\cite{keyulu2018jknet} 
uses dense residual connection at the last layer  
and combine all the intermediate representations nodewisely by different ways, 
including LSTM, Max-Pooling and so on. 

\textbf{MixHop}~\cite{abu2019mixhop} 
concats feature maps of several hops at each layer, represented as
\begin{equation*}
% \label{eq:ourlayer}
\mathbf{H}^{(\ell+1)} =\underset{j \in K}{\Bigg\Vert} \sigma\left(\tilde{\mathbf{P}}^j \mathbf{H}^{(\ell)} \mathbf{W}_j^{(\ell)}\right),  
\end{equation*}
which can be considered as staking several dense graph residual networks.   

% \subsubsection*{Dense Residues.}



% The models mentioned are listed as below:
% \begin{itemize}[leftmargin=4mm]
%     \item \textbf{APPNP}~\cite{klicpera2019appnp} (Initial Residue). 
%         \begin{equation*} 
%             \mathbf{H^{\ell+1}} = (1-\alpha) \tilde{\mathbf{P}}\mathbf{H^{\ell}} 
%             + \alpha \mathbf{H^{*}}. 
%         \end{equation*}
%     \item \textbf{GCNII}~\cite{chen2020gcnii}(Initial Residue). 
%      \begin{equation}
%         \label{eqn:gcnii_analysis}
%         \hspace{-0.7mm} \mathbf{H}^{(\ell+1)} \hspace{-0.7mm}= \hspace{-0.7mm}
%       \sigma  \hspace{-0.7mm}\left(  \hspace{-0.7mm}\left( \hspace{-0.5mm}  (1  \hspace{-0.7mm}-  \hspace{-0.7mm}\alpha_\ell)\tilde{\mathbf{P}}
%             \mathbf{H}^{(\ell)}  \hspace{-0.7mm} +  \hspace{-0.7mm}
%             \alpha_\ell\mathbf{H}^{*}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}
%           \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
%             \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right),
%         \end{equation}
%     \item \textbf{AIR}~\cite{zhao2021adaptive} (Initial Residue). 
        
%     \item \textbf{JKNet} (Dense Residue). 
% \end{itemize}

% \textbf{GCNII}\\
% \begin{equation}
%     \label{eqn:gcnii_analysis}
%     \hspace{-0.7mm} \mathbf{H}^{(\ell+1)} \hspace{-0.7mm}= \hspace{-0.7mm}
%   \sigma  \hspace{-0.7mm}\left(  \hspace{-0.7mm}\left( \hspace{-0.5mm}  (1  \hspace{-0.7mm}-  \hspace{-0.7mm}\alpha_\ell)\tilde{\mathbf{P}}
%         \mathbf{H}^{(\ell)}  \hspace{-0.7mm} +  \hspace{-0.7mm}
%         \alpha_\ell\mathbf{H}^{*}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}
%       \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
%         \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right),
% \end{equation}






==> Clenshaw Graph Neural Networks/www2023/3.2_Adaptive_initial_residue.tex <==
\subsection{Adaptive Initial Residue}
% \subsubsection*{\underline{Homophilic Assumption behind GCNII}}

The role of {\ul \textit{adaptive}} {\ul \textit{initial residue}} is to enable 
the expressive power of \textit{any} $K$-order polynomial filter.
To illustrate this, 
we will first consider an \textbf{incomplete} version of the ClenshawGCN termed HornerGCN. 

% \header{\bf Intuition of HornerGCN.}
\subsubsection*{\underline{Intuition}}
We start with an analysis of GCNII. 
To simplify the analysis, we consider 
$(1 - \beta_\ell) \mathbf{I}_n  +\beta_\ell \mathbf{W}^{(\ell)} $
as $\mathbf{I}$, 
and take $\textrm{relu}(x) = x$. 
At this point, the iteration~\eqref{eqn:gcnii_analysis} is simplified as
\begin{equation}
    \label{eqn:gcnii_analysis_simple}
    \hspace{-0.7mm} \mathbf{H}^{(\ell)} =
        (1  \hspace{-0.7mm}-  \hspace{-0.7mm}\alpha)\tilde{\mathbf{P}}
        \mathbf{H}^{(\ell-1)}  \hspace{-0.7mm} +  \hspace{-0.7mm}
        \alpha\mathbf{H}^{*}  .
\end{equation}

Consider a GCNII model of order $K$\footnote{For simplicity, we term a model 
with at most $K$ propagations as of order $K$}, 
by expanding \eqref{eqn:gcnii_analysis_simple},  
we obtain that 

\begin{equation}
    \label{eqn:gcnii_analysis_unfolded}
    \mathbf{H}^{(K)}= \sum_{\ell=0}^{K} \hat{\alpha}_{\ell} \tilde{\mathbf{P}}^{\ell} \mathbf{H}^{*}, 
\end{equation}
where 
$$
\hat{\alpha}_{\ell} =
\left\{\begin{matrix}
    \alpha(1-\alpha)^{\ell}, & \ell<  K, \\ 
     (1-\alpha)^{K}, & \ell = K.
\end{matrix}\right.
$$

It can be seen that the iterative process of GCNII 
implicitly leverages the representations of different layers 
with \textit{fixed} and \textit{positive} coefficients.  
However, we want \textit{flexible} exploitation of different diffusion layers, \cite{keyulu2018jknet,zhao2021adaptive}. 
More importantly, we need to have \textit{negative} weights 
in cases of heterophilic graphs \cite{chien2021gprgnn}.
To  this end, we can simply replace the fixed $\alpha$ in 
% \eqref{eqn:gcnii_analysis_simple} 
\eqref{eqn:gcnii_analysis}
with \textit{learnable} ones. 
In this way, we obtain
the form of HornerGCN
as follows,  

\begin{equation}
        \label{eq:horner_conv}
            \hspace{-0.7mm} \mathbf{H}^{(\ell)} \hspace{-0.7mm}= \hspace{-0.7mm}
           \sigma  \hspace{-0.7mm}
           \left(  \hspace{-0.7mm}
                \left(
                    \mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} 
                    +
                    \mymathhl{\alpha_{\ell}\mathbf{H}^{*}}
                \right)
                \hspace{-0.7mm}
              \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
                \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right),
\end{equation}
where $\ell = 0, 1, \ldots, K$, $\mathbf{H}^{(-1)}=\mathbf{O}$, 
$\mathbf{H}^{*} = \text{MLP}(\mathbf{X}; \mathbf{W^{*}})$.



% \header{\bf Spectral Nature.}
\subsubsection*{\underline{Spectral Nature}}
With the definition of \textit{polynomial filters} given in 
Equation~\eqref{eq:poly_filter_definition} and Definition~\ref{def:Polynomial Filters}, 
we will prove the Theorem below:
\begin{tcolorbox}[boxrule=0.2pt,height=40mm,boxrule=0.pt,valign=center,colback=blue!4!white]
    \begin{theorem}
    % [HornerGCN's corresponding polynomial filter]
    \label{thm:horner}
    A $K$-order HornerGCN 
    defined in Equation~\eqref{eq:horner_conv}, 
    when consider 
    $(1 - \beta_\ell) \mathbf{I}_n  +\beta_\ell \mathbf{W}^{(\ell)} $ for each $\ell$
    as 
    $\mathbf{I}$, 
    and $\textrm{relu}(x)$ as $x$, 
    simulates a \textit{polynomial filter} on the monomial basis: 
    % $$ 
    % h(\lambda) = \sum_{\ell=0}^{K}{\alpha}_{K-\ell} (1-\lambda)^{\ell},
    % $$ 
    
    $$ 
    h(\mu) = \sum_{\ell=0}^{K}{\alpha}_{K-\ell} \mu^{\ell},
    $$ 
    
    where $ \{\alpha_{\ell}\}_{\ell=0}^{K}$ is the set of 
    \textit{initial residue coefficients}.   
    \end{theorem}
\end{tcolorbox}

\subsubsection*{\underline{Horner's Method}}
To prove Theorem~\ref{thm:horner}, 
we first briefly introduce Horner's Method \cite{horner1819xxi}.
Given $p(x) = \sum_{i=0}^{n} a_i x^i = a_0 + a_1 x + \cdots a_n x^n$, 
Horner's Method is a classic method for evaluating 
$p(x_0)$, 
by  
% $$
%     p(x) = \sum_{i=0}^{n} a_i x^i = a_0 + a_1 x + \cdots a_n x^n
% $$, 
viewing  $p(x)$ as the following form:
\begin{align}
    \label{eq:horner_form}
    p(x)=a_0+x\left(a_1+x\left(a_2+x\left(a_3+\cdots+x\left(a_{n-1}+x a_n\right) \cdots\right)\right)\right) .
\end{align}

Thus, Horner's method defines a recursive method
for evaluating $p(x_0)$: 

% \begin{tcolorbox}[boxrule=0.2pt,height=32mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\begin{align}
    \label{eq:horner_recursive}
    b_n &:=a_n,  \nonumber \\
    b_{n-1} &:=a_{n-1}+b_n x_0, \nonumber  \\
    &\cdots  \nonumber  \\
    % b_1 &:=a_1+b_2 x_0 \\
    b_0 &:=a_0+b_1 x_0,  \nonumber  \\
    p(x_0) &:= b_0.
\end{align}


% \end{tcolorbox}

% \header{\bf HornerGCN.} 
\subsubsection*{\underline{Proof of Spectral Expressiveness}}
Note that the form of Horner's recursive 
are parallel with the recursive of stacked Horner convolutions by ignoring the non-linear transformations.
% simplifying $(1 - \beta_\ell) \mathbf{I}_n  +\beta_\ell \mathbf{W}^{(\ell)} $as $\mathbf{I}$
% and $\textrm{relu}(x)$ as $x$, 
% take the same simplicity as in \eqref{eqn:gcnii_analysis_simple} and 
Thus, by unfolding the nested expression of Horner convolutions \eqref{eq:horner_conv}, 
we get the output of the last layer closely matched with the form of Equation~\eqref{eq:horner_form} 
: 
% \begin{table}[H]
%     \centering
%     \begin{tcolorbox}[colback=white!1!white,height=60mm,boxrule=0.2pt,valign=center]
%         \textbf{HornerGCN Unfolded (With Adaptive Initial Residual)}
%             \begin{align*}
%             \label{eqn:horner_expansion_layerwise}
%             \hspace{-0.7mm} 
%             \mathbf{H}^{(0)} &= \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*},  \\
%             \mathbf{H}^{(1)} &= \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*}, \\
%             \mathbf{H}^{(2)} &= \tilde{\mathbf{P}}\left( \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*} \right) + \alpha_{2}\mathbf{H}^{*},\\
%             \cdots\\
%             \mathbf{H}^{(K)} 
%              &= \tilde{\mathbf{P}}\left(   \cdots  \tilde{\mathbf{P}}\left(   
%              \tilde{\mathbf{P}}
%                     \left(\alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*} \right) 
%                     + \alpha_{2}\mathbf{H}^{*} \right) \cdots + \alpha_{K-1}\mathbf{H}^{*} \right)  
%                     \\& \quad + \alpha_{K}\mathbf{H}^{*}
%                 \\
%                 &= \alpha_K\mathbf{H}^{*} + \alpha_{K-1} \tilde{\mathbf{P}} \mathbf{H}^{*} + \cdots + \alpha_{0} \tilde{\mathbf{P}}^{K} .
%             \end{align*}
%     \end{tcolorbox}
% \end{table}

% \begin{tcolorbox}[boxrule=0pt,height=58mm,boxrule=0pt,valign=center,colback=white!3!white]
% % \begin{tcolorbox}[title=HornerGCN Unfolded (With Adaptive Initial Residual),
%     % colback=blue!1!white,colframe=blue!20!black,
%     % boxrule=0.2pt,height=60mm,boxrule=0.3pt,valign=center] 
%     \begin{align}
%             \label{eqn:horner_expansion_layerwise}
%             \hspace{-0.7mm} 
%             \mathbf{H}^{(0)} &= \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*},  \nonumber \\
%             \mathbf{H}^{(1)} &= \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*}, 
%             \nonumber \\
%             \mathbf{H}^{(2)} &= \tilde{\mathbf{P}}\left( \alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*} \right) + \alpha_{2}\mathbf{H}^{*},
%             \nonumber \\
%             \cdots \nonumber \\
%             \mathbf{H}^{(K)} 
%              &= \tilde{\mathbf{P}}\left(   \cdots  \tilde{\mathbf{P}}\left(  
%              \tilde{\mathbf{P}}
%                     \left(\alpha_{0}\tilde{\mathbf{P}}\mathbf{H}^{*} + \alpha_{1}\mathbf{H}^{*} \right) 
%                     + \alpha_{2}\mathbf{H}^{*} \right) \cdots + \alpha_{K-1}\mathbf{H}^{*} \right)  
%                     \nonumber \\ 
%                     & \quad + \alpha_{K}\mathbf{H}^{*}
%                 \nonumber \\
%                 &= \alpha_K\mathbf{H}^{*} + \alpha_{K-1} \tilde{\mathbf{P}} \mathbf{H}^{*} + \cdots + \alpha_{0} \tilde{\mathbf{P}}^{K} 
%                 \nonumber \\
%                 &= \sum_{\ell=0}^{K} \alpha_{K-\ell} \tilde{\mathbf{P}}^{\ell} \mathbf{H}^{*}. 
%     \end{align}
% \end{tcolorbox}

% \begin{tcolorbox}[boxrule=0pt,height=45mm,boxrule=0pt,valign=center,colback=blue!3!white]
\begin{tcolorbox}[boxrule=0.2pt,height=45mm,boxrule=0.pt,valign=center,colback=blue!4!white]
% \begin{tcolorbox}[title=HornerGCN Unfolded (With Adaptive Initial Residual),
    % colback=blue!1!white,colframe=blue!20!black,
    % boxrule=0.2pt,height=60mm,boxrule=0.3pt,valign=center] 
    \begin{align}
            \label{eqn:horner_expansion_layerwise}
            \hspace{-0.7mm} 
            \mathbf{H}^{(0)} &= \alpha_{0}\mathbf{H}^{*},  \nonumber \\
            \mathbf{H}^{(1)} &= \tilde{\mathbf{P}} \left( \alpha_{0}\mathbf{H}^{*} \right)  + \alpha_{1}\mathbf{H}^{*}, 
            \nonumber \\
            % \mathbf{H}^{(2)} &=  \tilde{\mathbf{P}} \left( 
            %                                 \tilde{\mathbf{P}} \left( \alpha_{0}\mathbf{H}^{*} \right)  + \alpha_{1}\mathbf{H}^{*} 
            %                                 \right) + \alpha_{2}\mathbf{H}^{*},
            \cdots \nonumber \\ 
            \mathbf{H}^{(K)} &=  \tilde{\mathbf{P}} \left(  \cdots \left(
                            \tilde{\mathbf{P}} \left( 
                                            \tilde{\mathbf{P}} \left( \alpha_{0}\mathbf{H}^{*} \right)  + \alpha_{1}\mathbf{H}^{*} 
                                            \right) + \alpha_{2}\mathbf{H}^{*}
                            \right) \cdots \right) + \alpha_{K}\mathbf{H}^{*}
                            \nonumber \\
                            &= \alpha_K\mathbf{H}^{*} + \alpha_{K-1} \tilde{\mathbf{P}} \mathbf{H}^{*} + \cdots + \alpha_{0} \tilde{\mathbf{P}}^{K} 
                            \nonumber \\
                            &= \sum_{\ell=0}^{K} \alpha_{K-\ell} \tilde{\mathbf{P}}^{\ell} \mathbf{H}^{*}. 
    \end{align}
\end{tcolorbox}

% The expansion above is quite intuitive. In fact, 
% it adopts the matrix form of Horner's method \cite{horner1819xxi}. 
% More details of Horner's method could be found in the Appendix.
% The expansion \eqref{eqn:horner_expansion_layerwise} shows that,  
% by adding adaptive initial residues, 
% each level of fused representations can be leveraged. 

So, the final representation 
\begin{align*}
    \mathbf{H}^{(K)} &= 
\sum_{\ell=0}^{K} \alpha_{K-\ell} \tilde{\mathbf{P}}^{\ell} \mathbf{H}^{*}
= \mathbf{U} 
    \left(
        \sum_{\ell=0}^{K}{\alpha}_{K-\ell} \mathbf{M}^{\ell} 
    \right)
    \mathbf{U}^T \mathbf{H}^{*} ,
\end{align*}
corresponds to the result of 
a polynomial filter $h$ on the spectrum of $\mathbf{\tilde{P}}$, where 
% $b(\lambda)$ is
$$
    h(\mu) = 
    \sum_{\ell=0}^{K}{\alpha}_{K-\ell} \mu^{\ell}.
$$

% Note that Horner Convolution defined in \eqref{eq:horner_conv} 
% is equipped by only one of our proposed residual connections, 
% and is a \textbf{weakened version} of Clenshaw Convolution in \eqref{eq:clenshaw_conv}. 
% HornerGCN can be seen as simply a 
% \textit{recurring version of GPR} with transformation layers entangled 
% in each layer. 
% We take HornerGCN as an illustration for the use of Adaptive Initial Residue, 
% and it is an ablation model in the Experiment section.

% To be clear, we write the Horner's method as below: 
% \begin{theorem}[Horner's Method]
%     Given a polynomial $p(x)=\sum_{i=0}^{n}a_ix^i = a_0 + a_1 x  + \cdots a_n x^n $, 
%     where $a_0, \cdots, a_n $ are constant coefficients. \cdots
% \end{theorem}









==> Clenshaw Graph Neural Networks/www2023/3.3_Negative_residue.tex <==
\subsection{Negative Second Order Residue}
\label{sec:neg_residue}


The role of {\ul \textit{negative second order residue}} is to enable the leverage of Chebyshev basis. 
Compared with the adaptive initial residue, it is not obvious. 
In this section, we will first give an \textbf{intuitive} motivation 
for Negative Second Order Residue, 
and then reveal the mechanism behind it by Clenshaw Summation Algorithm.
% \textbf{graph polynomial filtering} under the Chebyshev basis.

% \subsubsection*{\underline{Spatial Intuition: Difference Relations}}
% \header{\bf Intuition of Taking Difference.} 
\subsubsection*{\underline{Intuition of Taking Difference}}
There is already some work that has noticed the `subtraction' relationship between progressive levels of representation~\cite{abu2019mixhop, Yang2022difference}. 
For example, one of MixHop's direct challenges towards the traditional GCN model is the inability to represent the \textit{Delta Operator}, \textit{i.e.}, 
% AX^2 - AX, 
$\mathbf{AX}^2\textcolor{red}{-}\mathbf{AX}$, 
which is an important relationship in representing both the concept of social boundaries~\cite{perozzi2018socialBoundary} and the concept of `sharpening' in images~\cite{burt1987laplacian, paris2011local}.

Instead of considering model's ability to represent \textit{Delta Operator} 
in the final output, 
we take a more direct use of these difference relations. 
That is, we add
$
\mymathhl{\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} -\mathbf{H}^{(\ell-2)}}
$
to \textit{each} convolution layers of \eqref{eq:horner_conv}, 
and get the final form of Clenshaw Convolution:
$$
\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} + \alpha_{\ell}\mathbf{H}^{*}
+ 
\mymathhl{\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} -\mathbf{H}^{(\ell-2)}} 
\Longrightarrow 
\eqref{eq:clenshaw_conv}.
$$

A question that perhaps needs to be answered is: why not instead 
insert a more direct difference relation: 
$
\underline{\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} -\mathbf{H}^{(\ell-1)}}
$
?
The reason is, 
at this point, the convolution would become
$$
\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} + \alpha_{\ell}\mathbf{H}^{*}
+ 
% \left(
\underline{\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} -\mathbf{H}^{(\ell-1)}}
% \right)
= 
\left(2\mathbf{\tilde{P}}-\mathbf{I}\right)\mathbf{H}^{(\ell-1)}
+ \alpha_{\ell}\mathbf{H}^{*},
$$
whose unfolded form, 
by substitute $\mathbf{\tilde{P}}$ to $2\mathbf{\tilde{P}}- \mathbf{I}$ in \eqref{eqn:horner_expansion_layerwise},  
would become $ \sum_{\ell=0}^{K} \alpha_{K-\ell} 
{\left(2\tilde{\mathbf{P}}-\mathbf{I}\right)}^{\ell} 
\mathbf{H}^{*}  $
, 
 which brings limited change.



\subsubsection*{\underline{Spectral Nature}}
% \header{\bf Spectral Nature.}
Besides the spatial intuition of considering substractions or boundaries, 
we reveal the spectral nature of our \textit{negative residual connection} in this part, that is, it simulates the leverage of chebyshev basis as in spectral polynomials.
With the definition of \textit{polynomial filters} given in 
Equation~\eqref{eq:poly_filter_definition} and Definition~\ref{def:Polynomial Filters}, 
% In this part,
we will prove the theorem below:
\begin{tcolorbox}[boxrule=0.2pt,height=45mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\begin{theorem}
    % [ClenshawGCN's corresponding polynomial filter]
    \label{thm:spatial_to_spectral}
    A $K$-order ClenshawGCN 
    defined in Equation~\eqref{eq:clenshaw_conv}, 
    when consider 
    $(1 - \beta_\ell) \mathbf{I}_n  +\beta_\ell \mathbf{W}^{(\ell)} $ for each $\ell$
    as 
    $\mathbf{I}$, 
    and $\textrm{relu}(x)$ as $x$, 
    simulates a \textit{polynomial filter} 
    $$ 
    h(\mu) = \sum_{\ell=0}^{K}{\alpha}_{K-\ell} U_{\ell}(\mu),
    $$ 
    where $ \{U_{\ell}\}_{\ell=0}^{K}$  is the truncated $K$-order  
    second-kind Chebyshev basis, 
    and $ \{\alpha_{\ell}\}_{\ell=0}^{K}$ is the set of 
    initial residue coefficients.   
    \end{theorem}
\end{tcolorbox}
which can also be expressed as:
\begin{align}
    \label{eq:hK}
    \mathbf{H}^{(K)} 
    = 
    \mathbf{U} 
    h({\mathbf{M}})
    \mathbf{U}^T \mathbf{H}^{*}
    = 
    \mathbf{U} 
    \left(
        \sum_{\ell=0}^{K}{\alpha}_{K-\ell} U_{\ell} (\mathbf{M}) 
    \right)
    \mathbf{U}^T \mathbf{H}^{*}.
\end{align}

\begin{comment}
\subsubsection*{\underline{Clenshaw Algorithm}}
For the proof of Theorem~\ref{thm:spatial_to_spectral}, 
we will first introduce Clenshaw Summation Algorithm 
% for the Second Kind of Chebyshev polynomials 
as a Corollary. 

\begin{tcolorbox}[boxrule=0.pt,height=60mm,boxrule=0.pt,valign=center,colback=blue!4!white]
   \begin{corollary}[Clenshaw Summation Algorithm for Chebyshev polynomials (Second Kind)]
    \label{cor:clenshaw}
    For the Second Kind of Chebyshev Polynomials, 
    the weighted sum of a finite series of $\{U_{k}(x)\}_{k=0}^{n}$ :
    \[
        S(x) = \sum_{k=0}^{k=n}\omega_k U_k(x) 
        \] 
    can be computed 
    by a recurrence formula:
    \begin{align}
        \label{eq:clenshaw_recurrence}
        b_{n+2}(x) &:= 0,  \nonumber
        \\
        b_{n+1}(x) &:= 0, \nonumber
        \\
        b_k(x) &:= \omega_k + 2x b_{k+1}(x) - b_{k+2}(x). \nonumber
        \\ &\quad\quad (k=n, n-1, ..., 0)
    \end{align} 
    Then $S(x) \equiv b_0(x)$.
\end{corollary}
\end{tcolorbox}


% \begin{corollary}[Clenshaw Summation Algorithm for Chebyshev polynomials (Second Kind)]
%     For the Second Kind of Chebyshev Polynomials, 
%     the weighted sum of a finite series of $\{U_{k}(x)\}_{k=0}^{n}$ :
%     \[
%         S(x) = \sum_{k=0}^{k=n}a_k U_k(x) 
%         \] 
%     can be computed 
%     by a recurrence formula:
%     \begin{align}
%         \label{eq:clenshaw_recurrence}
%         b_{n+2}(x) &:= 0,  \nonumber
%         \\
%         b_{n+1}(x) &:= 0, \nonumber
%         \\
%         b_k(x) &:= a_k + 2x b_{k+1}(x) - b_{k+2}(x), \nonumber
%         \\ &\quad\quad (k=n, n-1, ..., 0)
%         % \\ 
%         % S^*(x) &:= b_0(x)
%     \end{align} 
%     Then $S(x) == b_0(x)$.
% \end{corollary}

Clenshaw Summation can be applied to a wider range of polynomial basis. 
However, specifically for the second kind of Chebyshev, 
we made some slight simplifications\footnote{To be more precise, the simplification 
lies in that Clenshaw Summation procedures for the more general situation 
need an `extra' different step which is not needed in our proof.}, 
so for clarity of discussion, we give the proof here. 

\begin{proof}[Proof for Corollary~\ref{cor:clenshaw}]
Denote 
$$
A =  \begin{bmatrix}
            1 &  &  &  & \\  -2  & 1 &  &  & \\  1& -2 &1  &  & \\ 
             &  & \cdots &  & \\  &  &  1&  -2& 1 
    \end{bmatrix}, \quad
\vec{u} =   \begin{bmatrix}
                    U_{-1}(x)\\U_{0}(x)\\U_{1}(x)\\\cdots\\U_n(x)
            \end{bmatrix}, \quad
\vec{\omega} = \begin{bmatrix}
    0\\\omega_{0}\\\omega_{1}\\\cdots\\\omega_n
\end{bmatrix},
$$
with $A \in \mathbb{R}^{(n+2) \times (n+2)}$, $\vec{u} \in \mathbb{R}^{n+2}$, 
then   
\begin{align}
    \label{eq:s}
    S(x) =\vec{\omega}^T \vec{u}.
\end{align}
Indexing a vector from $-1$, 
we denote $\mathbf{1}_i \in \mathbb{R}^{(n+2)}$ as 
the one-hot vector with the $i$-th element being $1$ ($i$ starts from $-1$). 
Note that, since the recurrence relation for the Chebyshev polynomials~\eqref{eq:Urec},
\begin{align}
    \label{eq:cheb2-3-term}
    A \vec{u} =
    \begin{bmatrix}
    U_{-1}(x) \\ -2U_{-1}(x) + U_{0}(x) \\ 0 \\ \cdots \\ 0 
    \end{bmatrix}
    =
    \begin{bmatrix}
    0 \\ U_{0}(x) \\ 0 \\ \cdots \\ 0 
    \end{bmatrix}
    =
    % \begin{bmatrix} 0,&1,&0, &\cdots&0 \end{bmatrix}^T.
    \mathbf{1}_0.
\end{align}

% which is denoted as 
% $S(x) = \begin{bmatrix} 0&1&0 &\cdots&0 \end{bmatrix}^T$.  
Now suppose that there is a vector $\vec{b}  = [ b_{-1}, b_0, \cdots, b_n  ]$ 
satisfying 
\begin{align}
    \label{eq:suppose_b}
    \vec{\omega}^T = \vec{b}^TA ,
\end{align}
then 
$$
S(x) \stackrel{\eqref{eq:s}}{=} \vec{\omega}^T \vec{u} 
\stackrel{\eqref{eq:suppose_b}}{=} \vec{b}^TA\vec{u} 
\stackrel{\eqref{eq:cheb2-3-term}}{=} \vec{b} \mathbf{1}_0 = b_0.
$$
On the other hand, 
notice that the recurrence defined in \eqref{eq:clenshaw_recurrence} 
% is exactly the process of solving  $\vec{a}^T = \vec{b}^TA $ 
% iteratively from $b_n$ down to $b_0$, in a Gaussian Elimination form,
is exactly the Gaussian Elimination process of solving  $\vec{\omega}^T = \vec{b}^TA $ 
from $b_n$ down to $b_0$, 
which means that $\{b_n, \cdots, b_0\}$ calculated by \eqref{eq:clenshaw_recurrence}  
satisfies \eqref{eq:suppose_b}. Proof for Corollary~\ref{cor:clenshaw} is finished.
\end{proof}
\end{comment}


\subsubsection*{\underline{Clenshaw Algorithm}}
For the proof of Theorem~\ref{thm:spatial_to_spectral}, 
we will first introduce Clenshaw Summation Algorithm 
% for the Second Kind of Chebyshev polynomials 
as a Corollary. 

\begin{tcolorbox}[boxrule=0.pt,height=60mm,boxrule=0.pt,valign=center,colback=blue!4!white]
   \begin{corollary}[Clenshaw Summation Algorithm for Chebyshev polynomials (Second Kind)]
    \label{cor:clenshaw}
    For the Second Kind of Chebyshev Polynomials, 
    the weighted sum of a finite series of $\{U_{k}(x)\}_{k=0}^{n}$ :
    \[
        S(x) = \sum_{k=0}^{k=n}a_k U_k(x) 
        \] 
    can be computed 
    by a recurrence formula:
    \begin{align}
        \label{eq:clenshaw_recurrence}
        b_{n+2}(x) &:= 0,  \nonumber
        \\
        b_{n+1}(x) &:= 0, \nonumber
        \\
        b_k(x) &:= a_k + 2x b_{k+1}(x) - b_{k+2}(x). \nonumber
        \\ &\quad\quad (k=n, n-1, ..., 0)
    \end{align} 
    Then $S(x) \equiv b_0(x)$.
\end{corollary}
\end{tcolorbox}


% \begin{corollary}[Clenshaw Summation Algorithm for Chebyshev polynomials (Second Kind)]
%     For the Second Kind of Chebyshev Polynomials, 
%     the weighted sum of a finite series of $\{U_{k}(x)\}_{k=0}^{n}$ :
%     \[
%         S(x) = \sum_{k=0}^{k=n}a_k U_k(x) 
%         \] 
%     can be computed 
%     by a recurrence formula:
%     \begin{align}
%         \label{eq:clenshaw_recurrence}
%         b_{n+2}(x) &:= 0,  \nonumber
%         \\
%         b_{n+1}(x) &:= 0, \nonumber
%         \\
%         b_k(x) &:= a_k + 2x b_{k+1}(x) - b_{k+2}(x), \nonumber
%         \\ &\quad\quad (k=n, n-1, ..., 0)
%         % \\ 
%         % S^*(x) &:= b_0(x)
%     \end{align} 
%     Then $S(x) == b_0(x)$.
% \end{corollary}

Clenshaw Summation can be applied to a wider range of polynomial basis. 
However, specifically for the second kind of Chebyshev, 
we made some slight simplifications\footnote{To be more precise, the simplification 
lies in that Clenshaw Summation procedures for the more general situation 
need an `extra' different step which is not needed in our proof.}, 
so for clarity of discussion, we give the proof here. 

\begin{proof}[Proof for Corollary~\ref{cor:clenshaw}]
Denote 
$$
A =  \begin{bmatrix}
            1 &  &  &  & \\  -2x & 1 &  &  & \\  1& -2x &1  &  & \\ 
             &  & \cdots &  & \\  &  &  1&  -2x & 1 
    \end{bmatrix}, \quad
\vec{u} =   \begin{bmatrix}
                    U_{-1}(x)\\U_{0}(x)\\U_{1}(x)\\\cdots\\U_n(x)
            \end{bmatrix}, \quad
\vec{a} = \begin{bmatrix}
    0\\a_{0}\\a_{1}\\\cdots\\a_n
\end{bmatrix},
$$
with $A \in \mathbb{R}^{(n+2) \times (n+2)}$, $\vec{u} \in \mathbb{R}^{n+2}$, 
then   
\begin{align}
    \label{eq:s}
    S(x) =\vec{a}^T \vec{u}.
\end{align}
Indexing a vector from $-1$, 
we denote $\mathbf{1}_i \in \mathbb{R}^{(n+2)}$ as 
the one-hot vector with the $i$-th element being $1$ ($i$ starts from $-1$). 
Note that, since the recurrence relation for the Chebyshev polynomials~\eqref{eq:Urec},
\begin{align}
    \label{eq:cheb2-3-term}
    A \vec{u} =
    \begin{bmatrix}
    U_{-1}(x) \\ -2xU_{-1}(x) + U_{0}(x) \\ 0 \\ \cdots \\ 0 
    \end{bmatrix}
    =
    \begin{bmatrix}
    0 \\ U_{0}(x) \\ 0 \\ \cdots \\ 0 
    \end{bmatrix}
    =
    % \begin{bmatrix} 0,&1,&0, &\cdots&0 \end{bmatrix}^T.
    \mathbf{1}_0.
\end{align}

% which is denoted as 
% $S(x) = \begin{bmatrix} 0&1&0 &\cdots&0 \end{bmatrix}^T$.  
Now suppose that there is a vector $\vec{b}  = [ b_{-1}, b_0, \cdots, b_n  ]$ 
satisfying 
\begin{align}
    \label{eq:suppose_b}
    \vec{a}^T = \vec{b}^TA ,
\end{align}
then 
$$
S(x) \stackrel{\eqref{eq:s}}{=} \vec{a}^T \vec{u} 
\stackrel{\eqref{eq:suppose_b}}{=} \vec{b}^TA\vec{u} 
\stackrel{\eqref{eq:cheb2-3-term}}{=} \vec{b} \mathbf{1}_0 = b_0.
$$
On the other hand, 
notice that the recurrence defined in \eqref{eq:clenshaw_recurrence} 
% is exactly the process of solving  $\vec{a}^T = \vec{b}^TA $ 
% iteratively from $b_n$ down to $b_0$, in a Gaussian Elimination form,
is exactly the Gaussian Elimination process of solving  $\vec{a}^T = \vec{b}^TA $ 
from $b_n$ down to $b_0$, 
which means that $\{b_n, \cdots, b_0\}$ calculated by \eqref{eq:clenshaw_recurrence}  
satisfies \eqref{eq:suppose_b}. Proof for Corollary~\ref{cor:clenshaw} is finished.
\end{proof}


\subsubsection*{\underline{Proof of Spectral Expressiveness}} 
% In this part, we prove 
Now we prove Theorem~\ref{thm:spatial_to_spectral} inductively based on Corollary~\ref{cor:clenshaw}.
    
\begin{proof}[Proof of Theorem~\ref{thm:spatial_to_spectral}]
    \textbf{Given}: 
         \begin{equation}
    \label{eq:clenshaw_conv_linear}
             \mathbf{H}^{(\ell)} = 
                    2\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} 
                    {-\mathbf{H}^{(\ell-2)}} + {\alpha_{\ell}\mathbf{H}^{*}}, 
    \end{equation}
    $\mathbf{H}^{(-1)}=\mathbf{H}^{(-2)}=\mathbf{0}$.
    

    \textbf{Induction Hypothesis}: 
    Suppose that when the convolutions have processed to the $\ell$-th layer, 
    $\mathbf{H}^{(\ell-1)}$ and $\mathbf{H}^{(\ell-2)}$ 
    are already proved to be polynomial filtered results of $\mathbf{H}^{*}$,  
    % Denote their filtering functions as $h^{\ell-1}$ and $h^{\ell-2}$, respectively.
    we show that $\mathbf{H}^{(\ell)}$ is also polynomial filtered results of $\mathbf{H}^{*}$.
    
    Further, denote  the polynomial filtering functions
    of generating $\mathbf{H}^{(\ell-2)}$, $\mathbf{H}^{(\ell-1)}$ and $\mathbf{H}^{(\ell)}$ 
    to be  $h^{(\ell-2)}$,  $h^{(\ell-1)}$ and $h^{(\ell)}$.   
    Then $h^{(\ell)}$ satisfies:    
    \begin{align*}
        h^{(\ell)}(\mu) &= \alpha_{\ell} + 2\mu h^{(\ell-1)}(\mu) - h^{(\ell-2)}(\mu)   .
    \end{align*}

\textbf{Base Case}: 
For $\ell=0$, since $\mathbf{H}^{(-2)}=\mathbf{H}^{(-1)}=\mathbf{0}$, 
$ \mathbf{H}^{(0)} = \alpha_0 \mathbf{H}^{*}$, 
the first induction step is established with 
$$
h^{(0)}(\mu) = \alpha_0, 
\quad h^{(-1)}(\mu) = 0, 
\quad  h^{(-2)}(\mu) = 0.
$$

\textbf{Induction Step}: 
Insert
\begin{align*}
    \left\{\begin{matrix}
            \mathbf{H}^{(\ell-1)} 
                % &= \mathbf{U} h^{\ell-1}(\mathbf{\Lambda})\mathbf{U}^T\mathbf{H}^{*}
                &= \mathbf{U} h^{\ell-1}(\mathbf{M})\mathbf{U}^T\mathbf{H}^{*}
            , 
            \\
            \mathbf{H}^{(\ell-2)} 
                % &= \mathbf{U} h^{\ell-2}(\mathbf{\Lambda})\mathbf{U}^T\mathbf{H}^{*}
                &= \mathbf{U} h^{\ell-2}(\mathbf{M})\mathbf{U}^T\mathbf{H}^{*},
            \\
            \mathbf{\tilde{P}} 
                &=  \mathbf{U} \mathbf{M}\mathbf{U}^T 
\end{matrix}\right.
\end{align*}
into Equation~\eqref{eq:clenshaw_conv_linear}, we get 
     \begin{align*}
             \mathbf{H}^{(\ell)} &= 
                    2\underline{\mathbf{U} \mathbf{M}\mathbf{U}^T}
                    \dashuline{\mathbf{U} h^{(\ell-1)}(\mathbf{M})\mathbf{U}^T\mathbf{H}^{*}}
                    % \\&
                    - \dashuline{\mathbf{U} h^{(\ell-2)}(\mathbf{M})\mathbf{U}^T\mathbf{H}^{*}}
                    + {\alpha_{\ell}\mathbf{H}^{*}}
                    \\
                    &= \mathbf{U} \left(  
                    \alpha_{\ell} + 2\mathbf{M}h^{(\ell-1)}(\mathbf{M}) - h^{(\ell-2)}(\mathbf{M}) 
                    \right)
                    \mathbf{U}^T\mathbf{H}^{*}.
    \end{align*}
So, $\mathbf{H}^{(\ell)}$ is also a polynomial filtered result of $\mathbf{H}^{*}$, 
with filtering function $h^{(\ell)}$:  
\begin{align}
\label{eq:relation}
h^{(\ell)}(\mu) := \alpha_{\ell} + 2\mu h^{(\ell-1)}(\mu) - h^{(\ell-2)}(\mu)   .
% \\
% h^{(\ell)}(x) &:=  b^{(\ell)}(1-x). \nonumber
\end{align}

Stack relation\eqref{eq:relation} for $\ell=0,1,\cdots,K$, 
we get: 
\begin{align*}
    h^{(-2)}(\mu) &= 0, \\
    h^{(-1)}(\mu) &= 0, \\
    h^{(\ell)}(\mu) &:= \alpha_{\ell} + 2\mu h^{(\ell-1)}(\mu) - h^{(\ell-2)}(\mu), \quad
    \\ &\quad\quad 
    (k=0, 1, \cdots, K).
    % \\h^{(K)}(x) &:= b^{(K)}(1-x),
\end{align*}
where the progressive access of 
% each layer's coherent filtering function, 
% \textit{i.e.}
$b^{(\ell)}$ 
is in a \textbf{totally parallel} way with the recurrence \eqref{eq:clenshaw_recurrence} in Clenshaw Summation Algorithm. We soonly get 
$$
\sum_{\ell=0}^{K}{\alpha}_{K-\ell} U_{\ell} (\mu)  \equiv  h^{(K)}(\mu).
% ,\quad
% \sum_{\ell=0}^{K}{\alpha}_{K-\ell} U_{\ell} (1-\lambda) \equiv h^{(K)}(\lambda).
$$
% $$
% h^{K}(\lambda) = \sum_{\ell=0}^{K}{\alpha}_{K-\ell} U_{\ell} (1-\lambda).
% $$
Thus, we have finshed the proof of Theorem~\ref{thm:spatial_to_spectral}
.
\end{proof}



% \header{\bf Discussion.} 


==> Clenshaw Graph Neural Networks/www2023/3_Methodology.tex <==
\section{Method}
\label{sec:method}
\begin{comment}
\subsection{Residual Connections as Rewiring and Ensembling of Paths}
\textcolor{red}{Reference https://arxiv.org/pdf/1911.05722.pdf}
\\
To see where residual connection's power comes from, 
some works interpret ResNet\cite{He2016residual} as an \textit {ensemble} of many submodels\cite{Veit2016residual}, 
where each submodel is a \textit{path} that starts at the input and ends at the output. 
Correspondingly, in graph neural networks, 
such an \textit{ensemble} corresponds to 
a \textit{combination} of graph signals of different diffused levels.
% \textcolor{blue}{When building shortcuts in the message passing architecture, more }
This angle of view provides some explanation for existing residual connections.  
% and gives us a hint: 
% How to \textit{rewire} the model to introduce a good set of paths? 

\begin{figure}
\includegraphics[width=\columnwidth]{www2023/pics/path5.png}
% \includegraphics[width=\columnwidth]{www2023/pics/path6-1.png}
\caption{(Draft). In <UNNAMED MODEL>,  \textit{Paths} (marked by bold lines) constructed by residual connections  compose to Chebyshev polynomials of $\tilde{\mathbf{P}}$,   \textit{i.e.} 
% $\tilde{\mathbf{P}}$
$ U_1(\mathbf{\lambda}) = 4\lambda^2 -1 $ and 
$U_2(\mathbf{\lambda}) = 8\lambda^3 - 4\lambda$, respectively.
Note that \textit{transformation} operations in \textit{paths} are neglected.
}
% \Description{\textit{Paths} constructed in residual connections.}
\end{figure}

\subsubsection*{\textbf{Vanilla Residual Connections.}}
% This angle of view 
% provides some explanation of 
% why vanilla residual connections in GCN do bring not much benefit.
% $\cdots$ \textcolor{blue}{[quote figure]} \textcolor{blue}{[To state: Vanilla residue/Oversmooth]} 

\subsubsection*{\textbf{Initial Residual Connections.}}
% \textcolor{blue}{[Outline: Initial residue/Homophilic Hypothesis]}
% \textcolor{blue}
{GCNII's initial residue tilts all the ensembled paths to shorter or less diffused ones, which overcomes  over-smoothing. But it follows a homophily hypothesis.$\cdots$}

\subsubsection*{\textbf{Dense Residual Connections.}}

\subsubsection*{\textbf{Paths or Polynomials.}}
\textcolor{blue}{Polynomials of $\tilde{\mathbf{P}}$, 
or the ability to represent a certain polynomial of $\tilde{\mathbf{P}}$.}
\\ \\
\textcolor{blue}{First, the ensemble or composing of connections and paths, should not be too fixed to be expressive enough, 
nor too random to be accurate.-- The paths are composed corresponding to polynomial basis}
\\
\textcolor{blue}{Second, we want it to be neat in recurrence. Thus the model can be scalable.}
\\
\textcolor{blue}{We propose a residual connection mechanism with \textbf{an adaptive initial residue} and \textbf{a negative second order residue}.}
\end{comment}

\subsection{Clenshaw Convolution}

% First, recall the convolution from GCNII~\cite{chen2020gcnii}:
%      \begin{equation}
%         \label{eqn:gcnii_analysis}
%         \hspace{-0.7mm} \mathbf{H}^{(\ell+1)} \hspace{-0.7mm}= \hspace{-0.7mm}
%       \sigma  \hspace{-0.7mm}\left(  \hspace{-0.7mm}\left( \hspace{-0.5mm}  (1  \hspace{-0.7mm}-  \hspace{-0.7mm}\alpha_\ell)\tilde{\mathbf{P}}
%             \mathbf{H}^{(\ell)}  \hspace{-0.7mm} +  \hspace{-0.7mm}
%             \alpha_\ell\mathbf{H}^{*}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}
%           \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
%             \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right).
%         \end{equation}


% \header{\bf Clenshaw Convolution.}
We formulate the $\ell$-th layer's representation of ClenshawGCN as 
 \begin{equation}
    \label{eq:clenshaw_conv}
            \hspace{-0.7mm} \mathbf{H}^{(\ell)} \hspace{-0.7mm}= \hspace{-0.7mm}
           \sigma  \hspace{-0.7mm}
           \left(  \hspace{-0.7mm}
                \left(
                    2\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} 
                    % \underbrace{
                    \mymathhl{-\mathbf{H}^{(\ell-2)}}
                    % }_{\substack{\text{Negative Second} \\ \text{Order Residue}}}
                    + 
                    % \underbrace{
                    \mymathhl{\alpha_{\ell}\mathbf{H}^{*}}
                    % }_{test}
                \right)
                \hspace{-0.7mm}
              \left(  \hspace{-0.5mm}   (1  \hspace{-0.7mm} -  \hspace{-0.7mm}\beta_\ell) \mathbf{I}_n \hspace{-0.7mm} +
                \hspace{-0.7mm} \beta_\ell \mathbf{W}^{(\ell)}  \hspace{-0.7mm}\right)  \hspace{-0.7mm}\right),
        \end{equation}
where $\ell = 0, 1, \ldots , K$, $\mathbf{H}^{(-2)}=\mathbf{H}^{(-1)}=\mathbf{O}$, 
$\mathbf{H}^{*} = \text{MLP}(\mathbf{X}; \mathbf{W^{*}})$.

Note that 
for \textit{transformation}, we use identity mapping 
with $\beta_{\ell} = \log (\frac{\lambda}{\ell} + 1) \approx \lambda / \ell$
following GCNII~\cite{chen2020gcnii}. 
% and for \textit{propagation}, 
Comparing to GCNII, we include two simple yet effective residual connections: 
% we equip our convolution layer with two residual connections, 
\textbf{Adaptive Initial Residue} and \textbf{Negative Second Order Residue}:

 \begin{equation*}
        2\mathbf{\tilde{P}}\mathbf{H}^{(\ell-1)} 
        \underbrace{\mymathhl{-\mathbf{H}^{(\ell-2)}}}_{\substack{\text{
                    \textit{Negative} \underline{Second}} \\ \text{\underline{Order} Residue}}}
        + 
        \underbrace{\mymathhl{\alpha_{\ell}\mathbf{H}^{*}}
        .
        }_{ 
        \substack{
            \text{\textit{Adaptive}} \\ \text{\underline{Initial} Residue}
            }
        }
\end{equation*}

% Among the two residues, the role of the Adaptive Initial Residue is quite direct, 
% while the mechanism of the Negative Second Order Residue is not so obvious. 
% For the Negative Second Order Residue,
% besides introducing the spatial intuition of `differencing' or `sharpening',  
% we will give its coherent property as a spectral model. 


In the remaining part of this section, we will illustrate the role and mechanism of these two residual modules. 
In summary, 
\textit{adaptive initial residue} enables the simulating of any $K$-order polynomial filter, 
while \textit{negative second order residue}, 
motivated by the leveraging of `differencing relations', 
simulates the use of Chebyshev basis in the approximation of filtering functions.
For both two parts, 
we will give an intuitive analysis
with followed by a proofs.




% Note that, for the analysis below, 
% we apply an informal assumption following \cite{abu2019mixhop, chen2020gcnii}
% that 
% $$
% (1 - \beta_\ell) \mathbf{I}_n  +\beta_\ell \mathbf{W}^{(\ell)} 
% = \mathbf{I},
% \quad
% \textrm{relu}(x) = x.
% $$










==> Clenshaw Graph Neural Networks/www2023/4_Experiments.tex <==
\section{Experiments}
In this section, 
we conduct two sets of experiments with the node classification task. 
First, we verify the power of our method by comparing it with both spatial residual methods and powerful spectral models. 
Second, we verify the effectiveness of the two submodules by ablation studies. 
% \input{www2023/tables/fullsup_vs_res.tex}
% \input{www2023/tables/fullsup_vs_spectral.tex}

\subsection{Experimental Setup}
% \header{\bf Datasets and Splits.} 
\subsubsection*{\underline{Datasets and Splits}}



We use both homophilic graphs and heterophilic graphs in our experiments 
following former works, especially GCN~\cite{kipf2016semi}, Geom-GCN~\cite{Pei2020GeomGCN} and LINKX~\cite{Lim2021large}. 
\begin{itemize}[leftmargin= * ]
    \item \textit{Citation Graphs}.    
        Cora, PubMed, and CiteSeer are citation datasets~\cite{sen2008collective} 
        processed by Planetoid~\cite{yang2016revisiting}. 
        In these graphs, nodes are scientific publications, edges are citation links processed to be bidirectional, 
        and node features are bag-of-words representations of the documents. These graphs show strong homophily. 
    \item \textit{Wikipedia Graphs}. 
        Chameleon dataset and Squirrel dataset are page-page networks on topics in Wikipedia, 
        where nodes are entries, and edges are mutual links. 
    \item \textit{Webpage Graphs}. 
        Texas dataset and Cornell dataset 
        % are subsets from WebKB\footnote{http://www.cs.cmu.edu/afs/cs.cmu.edu/project/theo-11/www/wwkb}~\cite{craven1998learning}, 
        collect web pages from computer science departments of different universities. 
        The nodes in the graphs are web pages of students, projects, courses, staff or faculties~\cite{craven1998learning}, 
        the edges are hyperlinks between them, 
        and node features are the bag-of-words representations of these web pages. 
    \item \textit{Co-occurrence Network}. 
        The Actor network represents the co-occurrence of actors on a Wikipedia page~\cite{tang2009social}. 
        The node features are filtered keywords in the Wikipedia pages. 
        The categorization of the nodes is done by~\cite{Pei2020GeomGCN}.
    \item \textit{Mutual follower Network}. 
        Twitch-Gamers dataset represents the mutual following relationship between accounts on the streaming platform Twitch.  
\end{itemize}

We list the messages of these networks in Table~\ref{tbl:datasets}, where 
$\mathcal{H}(G)$ is the measure of homophily in a graph proposed by Geom-GCN~\cite{Pei2020GeomGCN}. 
Larger $\mathcal{H}(G)$ implies stronger homophily. 

\begin{table}[htp]
    \centering
    \caption{Statistics for the node classification datasets we use. 
    Datasets of different homophily degrees are used.  }
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{crrcc}
    \toprule
    Dataset       & \#Nodes       & \#Edges         & \#Classes &  $\mathcal{H}(G)$   \\ 
    \midrule
    Cora          & 2,709   & 5,429     & 7 &   .83   \\
    Pubmed        & 19,717  & 44,338    & 3 &   .71   \\
    Citeseer      & 3,327   & 4,732     & 6 &   .79   \\ 
    % \hline
    Squirrel      & 5,201   & 217,073   & 5 &  .22    \\
    Chameleon     & 7,600   & 33,544    & 5 &  .23    \\
    Texas         & 183     & 309       & 5 &  .11    \\
    Cornell       & 183     & 295       & 5 &   .30   \\
    Twitch-Gamers & 168,114 & 6,797,557 & 7 & .55 \\ 
    \bottomrule
    \end{tabular}
    \label{tbl:datasets}
    }
    \end{table}


% \header{\bf Experiment Setup.} 
% split & cross-validation
For all datasets except for the Twitch-gamers dataset, 
we take a 60\%/20\%/20\% train/validation/test split proportion 
following former works~\cite{Pei2020GeomGCN, chien2021gprgnn, He2021bern, he2022chebii}.
We run these datasets twenty times over random splits with random initialization seeds. 
For the Twitch-gamers dataset, 
we use the five random splits given in LINKX~\cite{Lim2021large} with a 50\%/25\%/25\% proportion
to align with reported results. 
% we take random splits with a 60\%/20\%/20\% train/validation/test proportion, 
% following former works~\cite{Pei2020GeomGCN, chien2021gprgnn, He2021bern, he2022chebii}, 
% We run experiments multiple times over the random split with random initialization seeds. 
% For the Twitch-gamers dataset, we use the random splits given in~\cite{Lim2021large} with a proportion of 50\%/25\%/25\% to align with reported results. 


% \header{\bf ClenshawGCN Setup.} 
\subsubsection*{\underline{ClenshawGCN Setup}}
Before and after the stack of Clenshaw convolution layers, 
two non-linear transformations are made to link with the dimensions of the raw features and final class numbers.     
All the intermediate transformation layers are set with 64 hidden units.  
For the initialization of the adaptive initial residues' coefficients, denoted as 
$\vec{\alpha} = \left[  \alpha_0, \cdots, \alpha_K \right]$, 
we simply set ${\alpha_K}$ to be $1$ and all the other coefficients to be $0$, 
which corresponds to initializing
% the coefficient of the $U_0$ to be $1$. 
% the initialization of
the polynomial filter to be $\mymathhl{g(\lambda) = 1}$ 
(or equivalently, $\mymathhl{h(\mu) = 1}$ ). 

% \header{\bf Hyperparameter Tuning.}
\subsubsection*{\underline{Hyperparameter Tuning}}
For the optimization process on the training sets, we tune $\vec{\alpha}$ with SGD optimizer with momentum~\cite{sutskever2013momentumImportance} 
and all the other parameters with Adam SGD~\cite{kingma2014adam}. 
We use early stopping with a patience of 300 epochs.

For the search space of hyperparameters, 
below is the search space of hyperparameters:
\begin{itemize}[leftmargin=7mm]
% \begin{itemize}
    \item Orders of convolutions: $K \in \left\{ 8, 12, \cdots, 32 \right\}$;
    \item Learning rates: $ \left\{ 0.001, 0.005,  0.1,  0.2,  0.3, 0.4, 0.5   \right\}$; 
    \item Weight decays: $\left\{ 1\mathrm{e}{-8}, 1\mathrm{e}{-7}, \cdots,  1\mathrm{e}{-3}   \right\}$;
    \item Dropout rates: $\left\{ 0,  0.1,  \cdots,  0.7   \right\}$.
\end{itemize}

We tune all the hyperparameters on the validation sets. 
To accelerate hyperparameter searching, we use Optuna~\cite{akiba2019optuna} and run 100 completed  
trials \footnote{
% For the term `trial':
In Optuna, a \textit{trial} means a run with hyperparameter combination; 
% For the term `':
the term `complete' refers to that, 
some trials of bad expectations would be pruned before completion.
% we use Optuna's MedianPruner to prune the trials of bad expectations
}
for each dataset. 


\subsection{Comparing ClenshawGCN with Other Graph Residual Connections} 
\input{www2023/tables/fullsup_vs_res.tex}
\input{www2023/tables/fullsup_vs_spectral.tex}
\label{sec:compare_residual}
In this subsection, we illustrate the effectiveness of ClenshawGCN's residual connections 
by comparing ClenshawGCN with other spatial models, including
% \header{\bf Baseline Models.} 
% We use the baseline models as follows:
GCNII~\cite{chen2020gcnii}, $\text{H}_2$GCN~\cite{zhu2020beyond}, 
MixHop~\cite{abu2019mixhop} and JKNet~\cite{keyulu2018jknet}. 
Among them, GCNII is equipped with initial residual connections, 
and the others are equipped with dense residual connections. 
Moreover, the way of combining multi-scale representations is more complex than weighted sum in $\text{H}_2$GCN and JKNet. 
As shown in Table~\ref{tb:full_residual}, our ClenshawGCN outperforms all the baselines. 
% Specifically, we outperform

On one hand, in line with our expectations, 
% by borrowing the strength from the spectral domain,  
ClenshawGCN outperforms all the baselines on the {\ul heterophilic datasets} by a significantly large margin 
including {\ul $\text{H}_2$GCN}, which is tailored for heterophilic graphs. 
This illustrates the effectiveness of borrowing spectral characteristics. 

% which demonstrates ClenshawGCN's ability in escaping from the homophily assumption. 
On the other hand, 
ClenshawGCN even shows an advantage over {\ul homophilic datasets}, 
though the compared spatial models, such as GCNII and JKNet, 
are strong baselines on such datasets. 
Especially, for the PubMed dataset, 
ClenshawGCN achieves state of art.   



\subsection{Comparing ClenshawGCN with Spectral Baselines} 
% We have seen from Section~\ref{sec:compare_residual} that by borrowing 
% Our model intend to establish connection to the characteristics of polynomial filters, 
% and 
% \input{www2023/tables/fullsup_vs_spectral.tex}
In Section~\ref{sec:neg_residue}, 
we have proved that ClenshawGCN acts as a spectral model
and simulates any $K$-order polynomial filter based on
% Chebyshev polynomial basis 
$\left\{U_{\ell}  \right\}_{\ell=0}^{\ell=K}$.
% of the second kind. 
In this subsection, we compare ClenshawGCN with strong spectral GNNs, 
including 
ChebNet~\cite{Defferrard2016cheb}, 
APPNP~\cite{klicpera2019appnp}, 
ARMA~\cite{bianchi2021arma}, 
GPRGNN~\cite{chien2021gprgnn}, 
BernNet~\cite{He2021bern}, 
and ChebNetII~\cite{he2022chebii}. 
Among them, APPNP simulates polynomial filters with \textit{fixed} parameters, 
ARMA GNN simulates ARMA filters~\cite{narang2013signalarma}, 
and the rest simulate \textit{learnable} polynomial filters based on the Chebyshev basis, Monomial basis or Bernstein basis. 

% As shown in Table~\ref{tb:full_residual}, our ClenshawGCN outperforms all the baselines. 

As reported in Table~\ref{tb:full_many}, 
ClenshawGCN outperforms almost all the baselines on each dataset, except for Chameleon and Citeseer. 
Specifically, ClenshawGCN outperforms other models on the Squirrel dataset 
by a large margin of $7.66\%$. 
% which uses cheby nodes interpolation

Note the comparison between ClenshawGCN and {ChebNetII}. 
ChebNetII gains \textit{extra power} from 
the leveraging of Chebyshev nodes, 
which is crucial for polynomial interpolation.   
% Chebyshev interpolation 
However, without the help of Chebyshev nodes,  
ClenshawGCN is comparable to ChebNetII in performance. 
The extra power of ClenshawGCN may come from the entangled non-linear transformations.



\subsection{Ablation Analysis}


\begin{figure}[htp]
    \includegraphics[width=\columnwidth]{www2023/pics/ablation.pdf}
    \caption{Results of the ablation study. HornerGCN and FixedParamClenshawGCN are weakened versions of ClenshawGCN. 
    HornerGCN is only equipped with adaptive initial residue, 
    and FixedParamClenshawGCN is only equipped with negative second-order residue. 
    The performance of these two ablation models are worse than a complete ClenshawGCN 
    but outperform GCN and GCNII.}
    \label{fig:ablation}
    \Description{figure description}
\end{figure}

For ClenshawGCN, the core of the design is the two residual connection modules. 
In this section, 
we conduct ablation analyses on these two modules to verify their contribution. 

% \header{\bf Ablation Model: HornerGCN.} 
\subsubsection*{\underline{Ablation Model: HornerGCN}}
We use HornerGCN as an ablation model to verify 
the contribution of \textit{negative residues}.
Recal Theorem~\ref{thm:horner}, 
the corresponding polynomial filter of HornerGCN is 
$$
    h_{Horner}(\mu) = \sum_{\ell=0}^{K}{\alpha}_{K-\ell} \mu^{\ell}, 
$$
which uses the Monomial basis. While the complete form of 
our ClenshawGCN borrows the use of chebyshev basis by negative residues.

% \header{\bf Ablation Model: FixedParamClenshawGCN.} 
\subsubsection*{\underline{Ablation Model: FixedParamClenshawGCN}}
In the FixedParamClenshawGCN model, 
we verify the contribution of \textit{adaptive} initial residue 
by fixing 
$\vec{\alpha} = \left[\hat{\alpha}_0, \hat{\alpha}_1, \cdots, \hat{\alpha}_K \right]$ with 
$$
    \hat{\alpha}_{\ell} = {\alpha}(1-{\alpha})^{K-\ell}, \quad \hat{\alpha}_{0} =(1-\alpha)^K  
$$
following APPNP~\cite{klicpera2019appnp}, 
where 
$ \alpha \in \left[ 0,1 \right] $ 
is a hyperparameter. 
The corresponding polynomial filter of FixedParamClenshawGCN is: 
$$
    h_{Fix}(\mu) = \sum_{\ell=0}^{K}{\hat{\alpha}}_{K-\ell} U_{\ell}(\mu).
$$


% \header{\bf Analysis.}  
\subsubsection*{\underline{Analysis}}
We compare the performance of HornerGCN and FixedParamClenshawGCN with 
GCN, GCNII and ClenshawGCN on two median-sized datasets: Chameleon and Squirrel. 
As shown in Figure~\ref{fig:ablation}, either removing the negative second-order residue 
or fixing the initial residue causes an obvious drop in Test Accuracy. 

Noticeably, 
% even equipped with only one of the two residual modules, 
with only one residual module, 
HornerGCN and FixedParamClenshawGCN still outperform 
homophilic models such as GCNII. 
For HornerGCN, the reason is obvious: HornerGCN simulates any polynomial filter, 
which is favorable for heterophilic graphs.   
For FixedParamClenshawGCN, though the coefficients of $U_{\ell}(\mu)$ are fixed, 
the contribution of each fused level (\textit{i.e.} $\mathbf{\tilde{P}^{\ell}}\mathbf{H}^{*}$) 
is no longer definitely to be \textit{positive} as in GCNII since each chebyshev polynomial 
consists of terms with \textit{alternating signs}, \textit{e.g.} $ U_4(\mathbf{\tilde{P}}) =  
16 \mathbf{\tilde{P}}^4 \textcolor{red}{-} 12 \mathbf{\tilde{P}}^2 \textcolor{red}{+} 1 $,  which  
breaks the underlying homophily assumption.




==> Clenshaw Graph Neural Networks/www2023/5_Discussions.tex <==
\section{Conclusion}
% This paper builds a connection 
In this paper, we propose 
ClenshawGCN, a GNN model equipped with a 
novel and neat residual connection module
% at each convolution layer
that is able to mimic a spectral polynomial filter. 
% By adding two residual connections 
When generating node representations for the next layer(\textit{i.e.} $\mathbf{H}^{(\ell+1)}$),
our model should only connect to the initial layer(\textit{i.e.} $\mathbf{H}^{(0)}$) \textit{adaptively},
and to the {second last layer}(\textit{i.e.} $\mathbf{H}^{(\ell-1)}$) \textit{negatively}.
% The way of $rewiring$ by residual connections
The construction of 
this residual connection inherently uses {Clenshaw Summation Algorithm}, 
a numerical evaluation algorithm for calculating weighted sums of Chebyshev basis. 
% in a \textit{recurrence} way.
We prove that 
our model 
implicitly simulates \textit{any} polynomial filter based on the \textit{second-kind Chebyshev basis} entangle with non-linear layers, bringing it at least comparable expressive power with state-of-art polynomial spectral GNNs.  
Experiments demonstrate our model's  superiority 
either compared with other spatial models with residual connections or with spectral models. 

For future work, 
a promising direction is to further investigate the 
mechanism and potential of such 
spectrally-inspired models entangled with non-linearity, 
which seems be able to incorporate the strengths of both sides.




==> Clenshaw Graph Neural Networks/www2023/tables/fullsup_vs_res.tex <==
% \subsection{Comparing clenshawNN with other residual-related methods.}
% \label{sec:compare_residual}
% Table~\ref{tb:full_residual} compares clenshawNN with other residual connection methods.

\begin{table*}[htp]
\centering
\small
\caption{
% Mean classification accuracy of full-supervised node classification with 60\%/20\%/20\% random splits.
Comparison with other models equipped by different kinds of residual connections.
Mean classification accuracies {(± standard derivation)}
of random splits are displayed. Besides the ClenshawGCN,
all the results are taken directly from \cite{Luan2021snowball} and \cite{Lim2021large}.
For the Twitch-Gamer dataset, we use 5 fixed 50\%/25\%/25\% splits
given in \cite{Lim2021large} to align with the reported results. 
For all the other datasets, 20 random 60\%/20\%/20\%  splits were used. 
(M) denotes some hyperparameter settings run out of memory \cite{Lim2021large}.
}
\resizebox{1.98\columnwidth}{!}{%
\begin{tabular}{@{}llllllllll@{}}
\toprule
% \begin{tabular}[c]{@{}l@{}}Datasets\\ \# Nodes\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Chameleon\\ 2,277\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Squirrel\\ 5,201\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Actor\\ 7,600\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Texas\\ 183\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Cornell\\ 183\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Cora\\ 2,708\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Citeseer\\ 3,327\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Pubmed\\ 19,717\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Twitch-gamer\\ 168,114\end{tabular} \\
  Datasets &Chameleon &Squirrel &Actor &Texas &Cornell & Cora & Citeseer & Pubmed & Twitch-gamer \\
  $|\mathcal{V}|$ &2,277 & 5,201 & 7,600 & 183  & 183 & 2,708 & 3,327 & 19,717 & 168,114\\
\midrule
{MLP} &
  46.59±1.84 &
  31.01±1.18 &
  40.18±0.55 &
  86.81±2.24 &
  84.15±3.05 &
  76.89±0.97 &
  76.52±0.89 &
  86.14±0.25 &
  60.92±0.07 \\
GCN &
  60.81±2.95 &
  45.87±0.88 &
  33.26±1.15 &
  76.97±3.97 &
  65.78±4.16 &
  87.18±1.12 &
  79.85±0.78 &
  86.79±0.31 &
  62.18±0.26 \\
\midrule
GCNII &
  63.44±0.85 &
  41.96±1.02 &
  36.89±0.95 &
  80.46±5.91 &
  84.26±2.13 &
  {\ul 88.46±0.82} &
  {\ul 79.97±0.65} &
  89.94±0.31 &
  63.39±0.61 \\
$\text{H}_2$GCN &
  52.30±0.48 &
  30.39±1.22 &
  {\ul 38.85±1.17} &
  {\ul 85.90±3.53} &
  {\ul 86.23±4.71} &
  87.52±0.61 &
  {\ul 79.97±0.69} &
  87.78±0.28 &
  (M) \\
MixHop &
  36.28±10.22 &
  24.55±2.60 &
  33.13±2.40 &
  76.39±7.66 &
  60.33±28.53 &
  65.65±11.31 &
  49.52±13.35 &
  87.04±4.10 &
  {\ul 65.64±0.27}\\
GCN+JK &
  64.68±2.85 &
  {\ul 53.40±1.90} &
  32.72±2.62 &
  80.66±1.91 &
  66.56±13.82 &
  86.90±1.51 &
  73.77±1.85 &
  {\ul 90.09±0.68} &
  {63.45±0.22} \\
% GAT+JK &
%   {\ul 68.14±1.18} &
%   52.28±3.61 &
%   35.41±0.97 &
%   75.41±7.18 &
%   74.43±10.24 &
%   {\ul 89.52±0.43} &
%   74.49±2.76 &
%   89.15±0.87 &
%   59.98±2.87 \\ 
  \midrule
ClenshawGCN &
  \textbf{69.44±2.06} & %0.92
  \textbf{62.14±1.65} &%0.70
  \textbf{42.08±1.99} &%0.86
  \textbf{93.36±2.35} &%0.99
  \textbf{92.46±3.72} &%1.64
  \textbf{88.90±1.26} &%0.59
  \textbf{80.34±1.26} &%0.57
  \textbf{91.99±0.41} & %0.17
  \textbf{66.26±0.27} \\ \bottomrule
\end{tabular}%
\label{tb:full_residual}
}
\end{table*}

==> Clenshaw Graph Neural Networks/www2023/tables/fullsup_vs_spectral.tex <==
% \subsection{Comparing clenshawNN with classic and strong baselines.}
% Table~\ref{tb:full_many} compares clenshawNN with some classic or strong baselines as in 
% ChebNetII an JacobiConv, to show that clenshawNN priors to both spatial and spectral methods.  

\begin{table*}[htp]
\centering

\small
\caption{
% ?Mean classification accuracy of full-supervised node classification with 60\%/20\%/20\% random splits.
Comparison with spectral models.
Mean classification accuracies {(±95\% confidence intervals)}
on 20 random 60\%/20\%/20\% train/validation/test splits are displayed. 
Besides the ClenshawGCN, 
all the results are taken directly from \cite{He2021bern}.
}

\resizebox{1.98\columnwidth}{!}{%
\begin{tabular}{@{}lllllllll@{}}
\toprule
  Datasets &Chameleon &Squirrel &Actor &Texas &Cornell & Cora & Citeseer & Pubmed \\
  $|\mathcal{V}|$ &2,277 & 5,201 & 7,600 & 183  & 183 & 2,708 & 3,327 & 19,717 \\
  \midrule

% \textcolor{blue}{MLP} &
%   46.59±1.84 &
%   31.01±1.18 &
%   40.18±0.55 &
%   86.81±2.24 &
%   84.15±3.05 &
%   76.89±0.97 &
%   76.52±0.89 &
%   86.14±0.25 \\
ChebNet &
  59.51±1.25 &
  40.81±0.42 &
  37.42±0.58 &
  86.28±2.62 &
  83.91±2.17 &
  87.32±0.92 &
  79.33±0.57 &
  87.82±0.24 \\
ARMA &
  60.21±1.00 &
  36.27±0.62 &
  37.67±0.54 &
  83.97±3.77 &
  85.62±2.13 &
  87.13±0.80 &
  80.04±0.55 &
  86.93±0.24 \\
APPNP &
  52.15±1.79 &
  35.71±0.78 &
  39.76±0.49 &
  90.64±1.70 &
  91.52±1.81 &
  88.16±0.74 &
  80.47±0.73 &
  88.13±0.33 \\
% \textcolor{blue}{TWIRLS} &
%   50.21±2.97 &
%   39.63±1.02 &
%   38.13±0.81 &
%   91.31±3.36 &
%   89.83±2.29 &
%   88.57±0.91 &
%   80.07±0.94 &
%   88.87±0.43 \\
% \textcolor{blue}{EGNN} &
%   51.55±1.73 &
%   35.81±0.91 &
%   35.16±0.64 &
%   81.34±1.56 &
%   82.09±1.16 &
%   87.47±1.33 &
%   80.51±0.93 &
%   88.74±0.46 \\
% PDE-GCN &
%   66.01±1.56 &
%   48.73±1.06 &
%   39.76±0.74 &
%   93.24±2.03 &
%   89.73±1.35 &
%   88.62±1.03 &
%   79.98±0.97 &
%   89.92±0.38 \\
GPRGNN &
  67.49±1.38 &
  50.43±1.89 &
  39.91±0.62 &
  92.91±1.32 &
  91.57±1.96 &
  88.54±0.67 &
  80.13±0.84 &
  88.46±0.31 \\
BernNet &
  68.53±1.68 &
  51.39±0.92 &
  41.71±1.12 &
  92.62±1.37 &
  92.13±1.64 &
  88.51±0.92 &
  80.08±0.75 &
  88.51±0.39 \\
ChebNetll &
  \textbf{71.37±1.01} &
  {\ul 57.72±0.59} &
  {\ul 41.75±1.07} &
  {\ul 93.28±1.47} &
  {\ul 92.30±1.48} &
  {\ul 88.71±0.93} &
  \textbf{80.53±0.79} &
  {\ul 88.93±0.29} \\
% JacobiConv &
%   \textbf{74.20±1.03} &
%   55.77±0.55 &
%   41.17±0.64 &
%   \textbf{93.44±2.13} &
%   \textbf{92.95±2.46} &
%   \textbf{88.98±0.46} &
%   \textbf{80.78±0.79} &
%   89.62±0.64 \\ 
  \midrule
ClenshawGCN &
  {\ul 69.44±0.92} & %0.92
  \textbf{62.14±0.70} &%0.70
  \textbf{42.08±0.86} &%0.86
  \textbf{93.36±0.99} &%0.99
  \textbf{92.46±1.64} &%1.64
  \textbf{88.90±0.59} &%0.59
  {\ul 80.34±0.57} &%0.57
  \textbf{91.99±0.17} \\ %0.17
  % \\
  \bottomrule
\end{tabular}%
\label{tb:full_many}
}
\end{table*}

==> www2023/1_intro_old.tex <==
\section{introduction}

\begin{figure}[htp]
\includegraphics[width=1.\columnwidth]{www2023/pics/residues.png}
\caption{figure caption}
\Description{figure description}
\end{figure}

% Over the past years, the study and design of neural networks on graph structures have become a popular topic.
The past few years have witnessed the rise of the graph learning field. 
In the graph learning field, 
% implicit or explicit 
relations (edges) between elements (nodes) are considered, 
\textit{e.g.} interactions among molecules[][], 
friendship or hostility between users[][],  
implicit syntactic or semantic structure in natural language[][]
and so on.
A paradigm of Graph Neural Networks was 
proposed in GCN\cite{kipf2016semi},  
% as an extreme simplification of 
which exploits the underlying graph topology 
by propagating node features iteratively along the edges. 
Along with the passing steps, 
information from a broader neighborhood is reached for each node. 
Such a \textit{propagation} entangled with non-linear \textit{transformation} 
forms a \textit{graph convolution layer} in GCN, 
denoted as $\mymathhl{f: x \to conv{(x)}}$.

However, just like what Convolution Neural Networks (CNNs) 
were faced with during its development[][], 
% GCN stacked by multiple convolution layers 
multi-stacked graph convolution layers
suffer from 
\textit{model degradation}[][]. 
Model degradation is the phenomenon 
when a model's performance come worse with a larger depth.  
% making it difficult for 
It hinders neural networks from 
the benefits of 
over-parameterization and large inceptions[][]. 


Model degradation of CNNs was solved by ResNet in the year of 2016\cite{He2016residual}.
% when He \textit{et. al.} raised \textit{residual connection}. 
This milestone module boosts CNNs in an extremely simple way: 
it only \textit{wraps} each convolution block with the $input$, 
denoted as $\mymathhl{f: x \to conv{(x) + x}}$
\footnote{Here, \textit{conv} is the convolution layer in CNN.}.


\textcolor{red}{[Recent works \& Perspective $\to$ Spectral Model]}\\
  
\begin{comment}
Following ResNet, 
researchers try to apply different residual connections  
to GCN[][][][][][][].
    \item \textbf{Raw Residual Connection}. 
    Early attempts[][] directly transplant 
    the \textit{raw residual connection} to GCNs, 
    % \textit{i.e.} $\mymathhl{f: x \to conv{(x)}+x}$, 
    but it doesn't work.   
    % The revelation of the cause  was achieved by
    The reason behind was gradually
    clarified with the discussion of \textit{over-smoothing}[][][]. 
    % Oversmoothing is the most discussed reason for the degradation of
    % GCNs, meaning that with features would be ...
    \item \textbf{Initial Residual Connection}. Along with the understanding of over-smoothing, \textit{initial residual connection} was proposed[] and explored with some variants[][]. However, despite of its ability to eliminate over-smoothing, 
    initial residual connection is only making a \textit{compromise} 
    between Laplacian smoothing and keeping identity, 
    which still follows the \textit{homophily assumption}[], 
    where each smoothed level of node features contributes \textit{positively}  
    to the final output.
    % that is, connected nodes tend to share similar features and labels. 
    More extensive use of different fused levels 
    is needed for non-homophily graphs[][]. 
    \item \textbf{Dense Residual Connections.} 
\end{comment}

Following ResNet, 
researchers try to apply different residual connections  
to GCN[][][][][][][].
Early attempts[][] directly transplant 
the \textit{raw residual connection} to GCNs, 
% \textit{i.e.} $\mymathhl{f: x \to conv{(x)}+x}$, 
but it doesn't work.   
% The revelation of the cause  was achieved by
The reason behind was gradually
clarified with the discussion of \textit{over-smoothing}[][][]. 

Along with the understanding of over-smoothing, 
\textit{initial residual connection} was proposed[] and explored with some variants[][]. 
% which can be roughly expressed as 
% $\mymathhl{f: x \to \alpha conv{(x) + \beta x^{*}}}$, 
% where $x^{*}$ is the initial representation of the node, 
% and $\alpha$ and $\beta$ are fixed[][] or not fixed. 
However, despite its ability to eliminate over-smoothing, 
initial residual connection is only making a \textit{compromise} 
between Laplacian smoothing and keeping identity, 
which still follows the \textit{homophily assumption}[], 
where each smoothed level of node features contributes \textit{positively}  
to the final output.
% that is, connected nodes tend to share similar features and labels. 
% It has been More extensive use of different fused levels 
% is needed for non-homophily graphs[][].  
Here comes our first motivation:
\begin{tcolorbox}[boxrule=0.pt,height=15mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\textbf{Motivation I}: Making flexible use of different 
fused levels of representations. 
\end{tcolorbox}
% \end{comment}

There are also \textit{denser residual connections} [][][]. 
Different from raw residual connection and initial residual connection 
that use \textit{only one} extra shortcut for each convolution layer, 
these models connect densely to the \textit{all} the former layers 
at the final step[] or at each intermediate step[][]. 
Some of these works do pull up the limit of expressive power that GNNs may reach[][], 
but their real actions are hard to analyze, 
and are often not very deep in use[][].

\begin{tcolorbox}[boxrule=0.pt,height=15mm,boxrule=0.pt,valign=center,colback=blue!4!white]
\textbf{Motivation II}: 
Constructing \textbf{neat} residual connections 
for easier analysis. 
\end{tcolorbox}

Though limited by the underlying homophily assumption, 
the progress made by initial residual connection 
gives a hint of making more use of graph topology. 
Over-smoothing is a GNN-specific cause of degradation.  







\textcolor{red}{[Our Model]}



When designing specific components, graph neural networks(GNNs) and general neural networks have both similar and special concerns. \textit{Residual connection}, what we are concerned about in this work, is such a component. 
Residual connection was first raised in ResNet\cite{He2016residual} to stack deep CNNs. 
It is famous for significant simplicity and strong ability in solving the \textit{model degradation} problem. 

On the other hand, there are causes of model degradation on the graph that are related to the topology of the graph, such as over-smoothing, which is different from the traditional model; 
in the work to be presented today, by constructing shortcuts, we can even bridge the connection between changing the path of information flow process and the graph Fourier and graph polynomial filters.



\\
\begin{comment}
    \textcolor{red}{[TODO: make the related work part more precise]}
\subsubsection*{\textbm{Residual Connections in Graph Learning}}
In the current literature, the following types of Residual Connection can be found: 
(1) one-hop to the previous layer; 
(2) one-hop to the initial layer; 
(3) densely connected to all the previous layers.

\subsubsection*{\underline{Residual Connection to the Previous Layer}}

In Vanilla GCN, each layer of convolution can be seen as a propagate of information on the graph.
This problem is known as oversmoothing, and is one of the more explored causes of GNN model degradation.
Vanilla GCN tries to connect to the Residual Connection of the previous layer, but the oversmoothing problem is still not solved: from the wandering point of view, connecting back to the Raw Residual Connection of the previous layer with $\alpha$.
is equivalent to turning a random walk into a lazy random walk.
The lazy random walk converges to the steady state (assuming the graph is connected and not bipartite), which corresponds to the principal eigenvector of the adjacency matrix.

\subsubsection*{\underline{Residual Connection to the Initial Layer}}

To alleviate the oversmoothing problem, the initial residual connection is connected back to the representation of the initial layer with a certain probability at each layer.
That is, the representation of the next layer is derived from the initial representation with a certain probability, instead of the neighborhood messages after multiple confusions.
This tilts a node's tendency towards maintaining its own feature against being over-smoothed.

It is noted in [] that initial Residual can be viewed as solving such an optimization problem: ( )(1).
The trade-off between multi-hop neighborhood information and initial features can also be seen in it.

In addition, there are variants of the Initial Residual Connection
AirGNN (GLASSO) takes a nodewise, sub-node form of $\alpha$ selection, but the essence of the solution is to use the Elastic Likelihood (ELL) method.
However, its essence is to solve the optimization problem improved by Elastic Lasso (1).
The object of its solution is still the homophiliy assumption.

Wentao Zhang et al. decoupled the Transformation and Propagation layers in the Convolution layer and adopted the Initial Residual Connection respectively, which is considered to solve the model degradation and over-smoothing problems, respectively.
The connection coefficients of Initial Residual are learned from the concatenation of the current layer and the initial layer.
However, it is still mainly applicable to homogeneous maps.

% Densely Forward Connected Residual Connection
\subsubsection*{\underline{Densely Connected Residual Connection
}}


Raw Residual Connection and Initial Residual Connection
both use some kind of single-line structure.
Some work suggests that displaying multiple representations of intermediate layers (i.e., feature maps for each level of confusion) simultaneously, 
and then selectively combining them with summation, max-pooling, concatenation, lstm, etc., to exploit more valid information (JKNet, MixHop). Theoretically, these works do pull up the upper limit of the expressive power that GNNs may reach, but these models are not very deep in use, and what is actually learned is not clear.

As another example, Li2019 tried a form of dense connectivity in DenseNet, but the space consumption associated with such connectivity is unaffordable.

In addition, work on polynomial filters on individual graphs also utilizes information from all intermediate layers in their implementation, including GPRGNN, ChebyNet, BernNet, etc. These works perform well on heterogeneous graphs, but formally, they differ significantly from Residual: they appear to be staked, whereas a work like ResNet is more like having a forward line with a more consistent iterative form.

\end{comment}


\subsubsection*{\textbf{Our Model}}

We introduced a new Residual Connection, which, unlike single-line connections and dense connections, has a two-line structure: the initial residual is simply a shortcuts to the upper layer, a change that keeps the structure of the model simple, but brings a Boost effect.

Why does this connection work so well?
First, it no longer follows the assumption of homogeneity, a consideration similar to that of GPRGNN, and what's more, its wiring (construction/rewiring) implicitly exploits the recursive relationship between Chebyshev bases, allowing for a more thorough exploitation of the layers - yes, just by a negative second shortcut. - The general idea behind this construction comes from a method that recursively evaluates the summation of polynomial bases: the Clenshaw algorithm.
This will be explained in detail in a later section. And we performed an ablation study to verify the effect of these two components.


\subsubsection*{\textbf{Deep or linear?}}

When ignoring linear transformation and activation together with propagation entangle, the model becomes a model on the spectral domain (linear GNN). However, we still choose an entangle together in such a way that it becomes a true `deep' model.

% Translated with www.DeepL.com/Translator (free version)


\newpage

